Secure Transfer Learning: Training Clean Models Against Backdoor in (Both) Pre-trained Encoders and Downstream Datasets

Transfer learning from pre-trained encoders has become essential in modern machine learning, enabling efficient model adaptation across diverse tasks. However, this combination of pre-training and downstream adaptation creates an expanded attack surface, exposing models to sophisticated backdoor embeddings at both the encoder and dataset levels--an area often overlooked in prior research. Additionally, the limited computational resources typically available to users of pre-trained encoders constrain the effectiveness of generic backdoor defenses compared to end-to-end training from scratch. In this work, we investigate how to mitigate potential backdoor risks in resource-constrained transfer learning scenarios. Specifically, we conduct an exhaustive analysis of existing defense strategies, revealing that many follow a reactive workflow based on assumptions that do not scale to unknown threats, novel attack types, or different training paradigms. In response, we introduce a proactive mindset focused on identifying clean elements and propose the Trusted Core (T-Core) Bootstrapping framework, which emphasizes the importance of pinpointing trustworthy data and neurons to enhance model security. Our empirical evaluations demonstrate the effectiveness and superiority of T-Core, specifically assessing 5 encoder poisoning attacks, 7 dataset poisoning attacks, and 14 baseline defenses across five benchmark datasets, addressing four scenarios of 3 potential backdoor threats.

==> sections/2-background.tex <==
\section{Background and Related Work}


\begin{figure}[!t]
\centering
\begin{minipage}[t]{0.23\textwidth}
\centering
\includegraphics[width=\textwidth]{images/threats/threat1.png}
\caption{Encoder Poisoning}
\label{fig:threat1}
\end{minipage}
\hfill
\begin{minipage}[t]{0.23\textwidth}
\centering
\includegraphics[width=\textwidth]{images/threats/threat2.png}
\caption{Dataset Poisoning}
\label{fig:threat2}
\end{minipage}
\hfill
\begin{minipage}[t]{0.23\textwidth}
\centering
\includegraphics[width=\textwidth]{images/threats/threat3.png}
\caption{Adaptive Poisoning}
\label{fig:threat3}
\end{minipage}
\hfill
\begin{minipage}[t]{0.23\textwidth}
\centering
\includegraphics[width=\textwidth]{images/threats/threat4.png}
\caption{Dual Poisoning}
\label{fig:threat4}
\end{minipage}
\caption{different threats}
\label{four threats}
\end{figure}


\subsection{Self-supervised Pre-training}\label{subsec:notations}
In this paper, we consider a popular transfer learning paradigm \cite{anton2022well,Ericsson2021HowTransfer} in image classification, \ie, "\textit{self-supervised pretraining} followed by \textit{supervised fine-tuning}".
The self-supervised stage is typically carried out by model service providers like Google and OpenAI who have sufficient computational power and access to a vast amount of unlabeled data, called \textit{pre-training dataset} $\predata$. The aim is to develop an image encoder serving as a representation function $g(\cdot; \theta): \mX \mapsto \mE$ using $\predata$, where $\mX = \R^d$ represents the input space, and $\mE$ is the embedding space.  
In the fine-tuning stage, a downstream user concatenates a task-specific classification head $f_\phi$ with parameters $\phi$ on top of the encoder $g$, creating a combined classification function $h (\cdot; \theta, \phi)=f\circ g: \mX \mapsto \Delta^{C}$, with $C$ being the number of classes and $\Delta^{C}$ representing the probability output space over the $C$ classes.
Taking advantage of the feature extraction capability of the encoder, the fine-tuning process primarily updates $\phi$ on the $C$-class labeled \textit{downstream training dataset} $\downdata$ with training loss $\sum_{(x_i, y_i) \in \downdata} \ell(h(x_i), y_i)$ between the probability of output $h(x)$ and $y$, while generally freezing or making minor adjustments to $\theta$. 
During inference, for any input feature $x \in \mathcal{X}$,  the resulting classifier $F(\cdot) := \argmax_c h_c(\cdot)$ takes $F(x)$ as the predicted label. The classifier is expected to have a high \textit{accuracy} (ACC) $\mathbb{E}_{(x,y) \sim \clean} \mathbb{I}(F(x) = y)$  on the clean data distribution $\clean$ of the downstream classification task.


% Self-supervised learning, as an emerging technique that enables models to learn generalizable representations from extensive unlabeled data, has become a popular prior choice to the transfer learning pipeline 
% After pre-training an image encoder using an unlabeled \textit{pre-training dataset}, it can be utilized to efficiently build models for various downstream tasks with labeled \textit{downstream dataset}.
% % Among many approaches to pre-train the encoder using unlabeled images, contrastive learning (\eg, SimCLR \cite{chen2020simple,chen2020big}, MoCo \cite{he2019moco,chen2020mocov2}) achieves the state-of-the-art performance for building downstream tasks.
% As a result, this \textit{self-supervised pre-training} followed by \textit{supervised fine-tuning}" paradigm is generally adopted in real-world applications. 
% The pre-training process is typically carried out by model service providers like Google and OpenAI, who have access to vast amounts of unlabeled data and computational power. The downstream users can leverage the released encoders from service providers to construct classifiers on their own tasks. 
% Therefore, this \textit{self-supervised pretraining} followed by \textit{supervised fine-tuning}" paradigm has become extremely popular.






\subsection{Backdoor Attacks}
\noindent \textbf{Backdoor Attacks in Supervised Learning.} 
Backdoor attack was first introduced in supervised classification task in BadNets is one of the earliest researches that performs backdoor attacks in DNNs. They injected several kinds of image pattern, referred to as the triggers, 178

R. Zheng et al.

into some samples, and modiﬁed the labels of the these samples to the desired malicious label. Then the DNNs were trained with the poisoned dataset and will be implanted a backdoor. After that, more covert and advanced backdoor designs were proposed [28,39,43]. To prevent defenders from reversely generating possible triggers through the model, dynamic backdoor attacks such as the InputAware Backdoor (IAB) [31], Warping-based Backdoor (WaNet) [30] and Sample Speciﬁc Backdoor Attack (SSBA) [24] were proposed. They generate a unique trigger for every single input, which makes the defense even more diﬃcult. These attacks can be classiﬁed as the poisoning based backdoor attacks.

Under some settings, it is also possible for the attackers to directly modify the architectures and parameters of a DNN, without poisoning any training data, known as the non-poisoning based backdoor attacks. For example, in Trojan attack [27], the triggers were optimized to increase the activation of some carefully chosen neurons, and then the network was retrained to ﬁnish the poisoning. In target bit trojan [33] and ProFlip [4], the authors choose vulnerable neurons and apply bit-ﬂip techniques to perform backdoor attacks. Note that, such bit ﬂip attack only occurs in the deployment phase of DNNs, and the ASR does not exceed other traditional ones. Therefore, this attack will not be discussed in this paper.


\noindent \textbf{Backdoor in Self-supervised Learning}

\subsection{Backdoor Defenses}
\textbf{Test-time Backdoor Detection}

\noindent \textbf{Training-time Defense} The training stage defenses aim at suppressing the eﬀect of implanted backdoor triggers or ﬁltering out the poisoned data during the training stage, with a full access to the training process. According to the diﬀerent distributions of poisoned data and clean data in feature space [18], several methods were proposed to ﬁlter out the poisoned data, including the robust statistics [13,38], input perturbation techniques [8,10] and semi-supervise training [18]. Besides, stronger data augmentation techniques [3] were proposed to suppress the eﬀect of backdoor, such as the CutMix [7], CutOut [7] and MaxUp [11]. Besides, diﬀerential privacy [9] and randomized smoothing [34] provide some certiﬁcated methods to defend against backdoor attack.

\noindent \textbf{Post-training Backdoor Removal}


% We use $\clean$ to denote the clean data distribution over $\mathcal{X} \times \{1,\dots,C\}$.

% \cite{chen2020simple}


==> sections/backup.tex <==
\appendices \label{Appendix}



\section{Implementations of Trusted Core}





\subsection{Full Algorithm} \label{Appendix:algo}

\begin{algorithm}[tbp]
\footnotesize
    \caption{ Trusted Core Bootstrapping}
    \label{algo:bootstrapping_learning}
    \KwIn{
    $g(\cdot; \prepara)$ (Untrusted encoder);
    \\\quad \quad \quad
    $\downdata$ (Untrusted downstream dataset);
    }
    % \KwOut{ $f_{\phi} \circ g(\cdot|\psi \cup \chi)$ (Clean classification model);}
    \KwOut{
    Trusted encoder 
    }
    \KwParam{
    $WarmupEpoch$ (Epoch number)
    \\  \quad \quad \quad  \quad \quad \quad 
    $\rho$ (filtered out data size);
    }
    \BlankLine

 % $\phi \leftarrow \textsc{RandomInitialize} (\phi$)\;        
% $\phi \leftarrow \textsc{Fine-tune} (\phi, \downdata) $\;      
Randomly initialize $\phi$\;
Train $\phi$ with  $\loss\Big( f_\phi \circ g(\cdot| \prepara), \cdot \Big)$ over $\cleandata$\;
$\seeddata \gets \textbf{Topological Invariance Sifting}\left( \prepara, D\right)$\;
$\subdata \gets \textbf{Seed Expansion} \left( \seeddata, \downdata \right)$\;
$\psi, \chi \gets \textbf{Encoder Channel Filtering}\left(\prepara, \downdata\right)$\;
Randomly initialize classifier head $\phi$ and untrusted neurons $\psi$\; 
\label{line:init_para}
$\cleandata \gets \subdata$\; \label{line:init_data}

    \For{$ i= 1$ to $Iter1$}{
    Train $\phi$ and $\psi$ using $\cleandata$ for $T$ epochs \;
        % $\phi \gets \min \frac{1}{|\cleandata|} \sum_{(x, y) \in \cleandata} \loss\left( f(\phi) \cdot g(x| \mathbf{m}^{\kappa}\odot \prepara), y\right)$\;
        Select $\gamma_1 \% $ samples with  the smallest loss from \textit{each class} of $\downdata \setminus \cleandata$ and add into $\cleandata$\; \label{line:add1}
    }

 \For{$ i= 1$ to $Iter2$}{
    Train $\phi$ and $\psi$ using $\cleandata$ for $T$ epochs \;
        Select $\gamma_2 \% $ samples with  the smallest loss from \textit{entire dataset} of $\downdata \setminus \cleandata$ and add into $\cleandata$\;  \label{line:add2}
    }


    \Repeat{ $|\cleandata| / |\downdata| \ge \rho $}{
        Train $\phi$ and $\psi$ with $\cleandata$ \;
        $\phi' \leftarrow \phi, \psi' \gets \psi $\;
        % \\
% $\phi', \psi' \leftarrow \max_{\phi', \psi'} \phi'-\beta \nabla_{{\phi}^{\prime}} \loss\left(f_{\phi'}\circ  g({x} | {\hat{\theta}}), y\right) $
         Train $\phi', \psi'$ using $\downdata\setminus\cleandata$ for one epoch \;
         $\mathtt{Loss}_1 \gets \{\loss(f(\phi) \circ g(x; \phi \cup \chi), y) \mid (x, y) \in \downdata \setminus \cleandata\}$\;
         $\mathtt{Loss}_2 \gets \{\loss(f(\phi') \circ g(x; \phi' \cup \chi), y) \mid (x, y) \in \downdata \setminus \cleandata\}$\;
         Select $\gamma_3\%$ samples with the lowest values in $\mathtt{Loss}_1 - \mathtt{Loss}_2$ and add them into $\cleandata$\; \label{line:add3}
    }
    
    % \For{$i = 1$ to $MetaEpoch$}{
    %     Train $\phi$ and $\psi$ with \cref{eq:learn_and_unlearn}\;
    %      Obtain $\phi'$ from \cref{eq:meta_phi} using $\phi$ and $\downdata\setminus\cleandata$ \;
    %      $\mathtt{Loss}_1 \gets \left\{ \loss\left(f_\phi\circ g(x|\hat{\theta}), y\right) \Big| (x, y) \in \downdata \setminus \cleandata \right\}$\;
    %      $\mathtt{Loss}_2 \gets \left\{ \loss\left(f_{\phi'}\circ g(x|\hat{\theta}), y\right) \Big| (x, y) \in \downdata \setminus \cleandata \right\}$\;
    %      Select $\gamma_2$ samples with the lowest values in $\mathtt{Loss}_1 - \mathtt{Loss}_2$ and add them into $\cleandata$\;
    % }
    
    
    % \textbf{Optimize network structure}
    % Apply CLP BN and filter to (encoder + classifier $C_0$)\;
    % Fine-tune BN and filter using $\mathcal{D}_{clean}$\;
    \Return{$\phi, \psi, \chi$}

\label{algo:entire}
\end{algorithm}





In \cref{algo:bootstrapping_learning}, we present the overall pipeline of our Trusted Core Bootstrapping framework, as well as the algorithmic details we introduced in \cref{sec:bootstrapping}.







\subsection{Details of Each Module}
\noindent\textbf{Details of Topological Invariance Sifting.}
% \subsubsection{Details of Topological Invariance Sifting}
The algorithm  \cref{algo:sifting} in \cref{sec:seedsifting} extracts high-credibility seed data from a poisoned dataset by utilizing topological invariance across various layers of a well-trained poisoned model.
For clustering, we employ activations from the output of the encoder and the first two layers of the classifier, and implement density-based clustering using DBSCAN \cite{ester1996density}.
We set the number of nearest neighbors \( m \) to 50 and employ Euclidean distance for neighbor determination. The seed selection ratio \( \alpha \) is set to 1\%.

\noindent\textbf{Details of Seed Expansion}
% \subsubsection{Details of Seed Expansion}
\cref{algo:seedexpansion} in \cref{sec:data_expansion} expand the seed data obtained from \cref{algo:sifting}.
We set the select ratio $r_\textrm{expand}$ for expansion as 5\%, and the expansion ratio \( |\subdata| / |\downdata|\) as 10\%.


\noindent\textbf{Details of Encoder Channel Filtering}
% \subsubsection{Details of Encoder Channel Filtering}
The algorithm in \cref{algo:pruning} from \cref{sec:encoder_filtering} filters trusted and untrusted channels within the pre-trained encoder. The unlearning process stops once the training accuracy drops below 20\%. The recovery process is conducted using the Adam optimizer with a learning rate of 0.01. Training is performed for 120 epochs. The filtering threshold is set to cut off 10\% of channels as untrusted.

\noindent\textbf{Details of Clean Bootstrapping Training}
% \subsubsection{Details of Clean Bootstrapping Training}
The clean bootstrapping described in \cref{algo:bootstrapping_learning} iteratively expands the clean subset and refines the model parameters. We set both \( Iter1 \) and \( Iter2 \) to 10, with both \( \gamma_1\% \) and \( \gamma_2\% \) set to 2\%. Additionally, \( \gamma_3\% \) is set to 5\%. This process continues until the clean subset reaches \( \rho = 90\% \) of the entire dataset.






\section{Experimental Setup Explanation} \label{sec:implementation_details}


\subsection{Datasets Explanation} \label{sec:dataset_explanation}
We detail the datasets utilized and how we process them as pre-training or downstream datasets as follows:
\begin{itemize}[leftmargin=6pt]

\item {\bf STL-10~\cite{coates2011analysis}:} 
The STL-10 dataset comprises 5,000 labeled training images, 8,000 labeled testing images, and an additional 100,000 unlabeled images, each with dimensions of 96 $\times$ 96 $\times$ 3, and all parts of the image set can be evenly divided into ten classes, where each image belongs to one category. We use the 100,000 unlabeled images for the pre-training dataset and the labeled part for the downstream training and testing.

\item {\bf CIFAR-10~\cite{krizhevsky2009learning}:} This dataset is also a balanced dataset containing 50,000 labeled training images and 10,000 testing images, both of which are evenly divided into 10 classes. Each image has a size of 32$\times$32$\times$3. We use this dataset for the downstream dataset and remove the labels of the training images when pre-training the encoder.



\item {\bf GTSRB~\cite{stallkamp2012man}:} This dataset contains 43 classes of traffic signs, split into 39,209 training images and 12,630 test images. Each image has a size of 32$\times$32$\times$3. Furthermore, this dataset has an uneven distribution of the number of images belonging to each class, ranging from 210 to 2250, which presents a real-world challenge, especially when under poisoning. Thus, we use it for the downstream dataset to evaluate the effectiveness of defenses.

\item {\bf SVHN~\cite{netzer2011reading}:} In this dataset, every image depicts a digit from the house numbers collected from Google Street View with the size of 32$\times$32$\times$3. Additionally, the images fall into one of the ten possible digit categories. 
There are 73,257 training images and 26,032 testing images in this dataset. Moreover, extraneous digits are added at the edges of the primary digit in focus, making it even more challenging to separate poisoned and clean samples under SVNH. Thus, we also use it as a downstream dataset to test the robustness of defenses.

\item {\bf ImageNet~\cite{deng2009imagenet}:} This dataset is built for large-scale object classiﬁcation and contains 1,281,167 training samples and 50,000 testing samples in 1000 classes. The input size is 224$\times$224$\times$3.
We use a 100-class subset for the pre-training dataset and a 10-class subset for the downstream dataset to evaluate our defense's scalability.


\end{itemize}





\vspace{-2mm}
\subsection{Pre-trained Encoder Explanation}\label{subsec:EncoderExplanation}
\vspace{-2mm}
Here, we provide the details of each encoder poisoning attack,  how we obtain both these clean and poisoned encoders, and how we use them to process transfer learning.

\noindent \textbf{BadEncoder} and \textbf{DRUPE}: Both methods inject backdoors by fine-tuning a clean pre-trained encoder, assigning a target class to a specific concept in a downstream dataset. 
Our experiments are conducted by using STL-10 as a pre-training dataset with backdoors targeting CIFAR-10, GTSRB, and SVHN, as well as CIFAR-10 as a pre-training dataset targeting STL-10, GTSRB, and SVHN.

\noindent \textbf{CTRL}: Different from the way of injecting the backdoor of BadEncoder and DRUPE, CTRL contaminates the unlabeled images in the pre-training dataset, targeting a concept within the label set of this pre-training dataset. 
Consequently, its backdoor only functions on downstream datasets with the same or a subset of the pre-training dataset's label set.
Thus, we follow \cite{CTRL} and use CIFAR-10, STL-10, and GTSRB, each as both pre-training and downstream datasets. 

\noindent \textbf{SSLBackdoor} and \textbf{CorruptEncoder}: Both methods use the same 100-class subset of ImageNet as the pre-training dataset, injecting backdoors similarly to the CTRL method by directly poisoning the pre-training data. We use a 10-class subset of ImageNet as the downstream dataset, ensuring that the target classes of both SSLBackdoor and CorruptEncoder are included in this subset. 
% Note that we also evaluate a variant of CorruptEncoder, denoted as CorruptEncoder++.


Additionally, for the clean encoder of STL-10 and CIFAR-10, we follow \cite{BadEncoder} to use SimCLR to train a ResNet18 using the publicly available code of SimCLR\footnote{\href{https://github.com/leftthomas/SimCLR}{https://github.com/leftthomas/SimCLR}}.
The clean ImageNet encoder are provided by \cite{SSL-backdoor}\footnote{\href{https://github.com/UMBCvision/SSL-Backdoor}{https://github.com/UMBCvision/SSL-Backdoor}}.
The backdoor encoders are constructed through each backdoor poisoning method.
For BadEncoder\footnote{\href{https://github.com/jinyuan-jia/BadEncoder}{https://github.com/jinyuan-jia/BadEncoder}} and DRUPE\footnote{\href{https://github.com/Gwinhen/DRUPE}{https://github.com/Gwinhen/DRUPE}}, we directly use their open-source checkpoints trained on STL-10 and CIFAR-10.
For the ImageNet backdoor encoder, we use the checkpoints provided by \cite{zhang2022corruptencoder}\footnote{\href{https://github.com/jzhang538/CorruptEncoder}{https://github.com/jzhang538/CorruptEncoder}} for SSL-Backdoor and CorruptEncoder.



\subsection{Dataset Poisoning Explanation} \label{subsec:DatasetPoisoningExplanation}
For dataset backdoor poisoning,  we use the  backdoor-toolbox\footnote{\href{https://github.com/vtu81/backdoor-toolbox}  {https://github.com/vtu81/backdoor-toolbox}} benchmark to implement all the attacks on downstream datasets.
Note that this benchmark does not provide experimental setups for certain attack methods on some datasets. For instance, TaCT attack on ImageNet is originally not supported. We conducted experiments by adapting the settings from other datasets.
\\
\noindent
\textbf{Trigger and Target Class.}
In the context of \threattwo, we employed distinct triggers and target classes to avoid conflicts between Encoder Poisoning and Dataset Poisoning. Specifically, when both \threatone~ and \threattwo~ are present, we maintained the same approach used for \threattwo.
In \threatthree, we utilized the same triggers and target classes as those applied in the pre-trained encoder.
For \threattwo, aside from TaCT, the target classes are as follows: ``Car'' for STL-10, ``Bird'' for CIFAR-10, ``Speed limit (50km/h)'' for GTSRB, ``2'' for SVHN, and ``n01855672 (Goose)'' for ImageNet-10. The specific target classes for TaCT and \threatthree~ across various datasets are detailed in \cref{tab:target_class}.
\\
\noindent
\textbf{Poisoning and Cover Ratio.}
By default, the poisoning rate was set to 20\% of the target category. For specific attacks like TaCT, WaNet, Adap-Blend, and Adap-Patch, the cover rate was set to 1/4 of the poisoning rate.
\begin{table}[ht]
    \caption{Target Class of Various  Dataset Poisoning Methods on Downstream Dataset}
    \adjustbox{center}{
        \resizebox{0.49\textwidth}{!}{\Huge
        \setlength{\tabcolsep}{0.6pt}
        \begin{tabular}{c|ccc|ccc}
        \toprule
        \rowcolor[HTML]{CCCCCC} 
        \textbf{Threat Type} & \multicolumn{3}{c|}{\cellcolor[HTML]{CCCCCC}\textbf{Threat 2}} & \multicolumn{3}{c}{\cellcolor[HTML]{CCCCCC}\textbf{Threat 3}} \\ \midrule
        \rowcolor[HTML]{D9D9D9} 
        \cellcolor[HTML]{D9D9D9} & \multicolumn{3}{c|}{\cellcolor[HTML]{D9D9D9}TaCT} & \multicolumn{1}{c|}{\cellcolor[HTML]{D9D9D9}BadEncoder} & \multicolumn{1}{c|}{\cellcolor[HTML]{D9D9D9}DRUPE} & CTRL \\ \cline{2-7} 
        \rowcolor[HTML]{D9D9D9} 
        \multirow{-2}{*}{\cellcolor[HTML]{D9D9D9}Dataset} & \multicolumn{1}{c|}{\cellcolor[HTML]{D9D9D9}Target Class} & \multicolumn{1}{c|}{\cellcolor[HTML]{D9D9D9}Source Class} & Cover Class & \multicolumn{1}{c|}{\cellcolor[HTML]{D9D9D9}Target Class} & \multicolumn{1}{c|}{\cellcolor[HTML]{D9D9D9}Target Class} & Target Class \\ \midrule
        STL-10 & \multicolumn{1}{c|}{Car} & \multicolumn{1}{c|}{Truck} & Dog Horse Monkey & \multicolumn{1}{c|}{Trunk} & \multicolumn{1}{c|}{Trunk} & Airplane \\ \midrule
        CIFAR-10 & \multicolumn{1}{c|}{Bird} & \multicolumn{1}{c|}{Truck} & Dog Forg Horse & \multicolumn{1}{c|}{Airplane} & \multicolumn{1}{c|}{Airplane} & Airplane \\ \midrule
        GTSRB & \multicolumn{1}{c|}{Speed limit (60km/h)} & \multicolumn{1}{c|}{Speed limit (50km/h)} & \begin{tabular}[c]{@{}c@{}}Speed limit (50km/h)\\ End of speed limit(80km/h)\\ Speed limit(100km/h)\end{tabular} & \multicolumn{1}{c|}{Priority Road} & \multicolumn{1}{c|}{Priority Road} & Speed limit(20km/h) \\ \midrule
        SVHN & \multicolumn{1}{c|}{2} & \multicolumn{1}{c|}{1} & 5 6 7 & \multicolumn{1}{c|}{0} & \multicolumn{1}{c|}{0} & None \\ \midrule
        \rowcolor[HTML]{D9D9D9} 
        \cellcolor[HTML]{D9D9D9} & \multicolumn{3}{c|}{\cellcolor[HTML]{D9D9D9}TaCT} & \multicolumn{1}{c|}{\cellcolor[HTML]{D9D9D9}SSLBackdoor} & \multicolumn{1}{c|}{\cellcolor[HTML]{D9D9D9}CorruptEncoder} & - \\ \cline{2-7} 
        \rowcolor[HTML]{D9D9D9} 
        \multirow{-2}{*}{\cellcolor[HTML]{D9D9D9}Dataset} & \multicolumn{1}{c|}{\cellcolor[HTML]{D9D9D9}Target Class} & \multicolumn{1}{c|}{\cellcolor[HTML]{D9D9D9}Source Class} & Cover Class & \multicolumn{1}{c|}{\cellcolor[HTML]{D9D9D9}Target Class} & \multicolumn{1}{c|}{\cellcolor[HTML]{D9D9D9}Target Class} & - \\ \midrule
        ImageNet-10 & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}n01855672\\ (Goose)\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}n01775062\\ (Wolfspider)\end{tabular}} & \begin{tabular}[c]{@{}c@{}}n02120079(Whitefox)\\ n02447366(Badger)\\ n02483362(Gibbon)\end{tabular} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}n02116738\\ (Hunting Dog)\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}n02116738\\ (Hunting Dog)\end{tabular}} & \begin{tabular}[c]{@{}c@{}}-\end{tabular} \\ \bottomrule
        \end{tabular}
        }
    }
    \vspace{-2mm}
    \label{tab:target_class}
    \end{table}




\subsection{Baseline Defense Explanation}
\noindent


In our evaluation of baseline defense, we tailor all the end-to-end training from scratch to transfer learning using a clean or poisoned encoder based on the specific threat.
We utilize the publicly available code of \cite{qi_sec_2023}\footnote{\url{https://github.com/Unispac/Fight-Poison-With-Poison}} to implement STRIP, AC, Spectral, SPECTRE, and CT. 
We utilize the toolbox\footnote{\url{https://github.com/THUYimingLi/BackdoorBox}} to implement IBD-PSC and SCALE-UP.
We implement ASSET\footnote{\url{https://github.com/reds-lab/ASSET}}, 
ABL\footnote{\url{https://github.com/bboylyg/ABL}}, CBD\footnote{\url{https://github.com/zaixizhang/CBD}}, 
CLP\footnote{\url{https://github.com/rkteddy/channel-Lipschitzness-based-pruning}},
SSLBackdoorMitigation\footnote{\url{https://github.com/wssun/SSLBackdoorMitigation}},
META-SIFT\footnote{\url{https://github.com/ruoxi-jia-group/Meta-Sift}}, 
FT-SAM\footnote{\url{https://github.com/SCLBD/BackdoorBench}},
and I-BAU\footnote{\url{https://github.com/YiZeng623/I-BAU}} using their respective official code repositories.
Particularly, the original CLP only exerts on the convolution layer of the encoder, we also prune the classification head after the backdoor injection of downstream dataset poisoning.






% For poison removal, we implement CLP on the encoder using its official implementation \footnote{\href{https://github.com/rkteddy/channel-Lipschitzness-based-pruning}{https://github.com/rkteddy/channel-Lipschitzness-based-pruning}}, and tailor the implementation to MLP based on its logical structure when  
% For distillation, we implemented  following their official open-sourced code SSLBackdoorMitigation\footnote{\href{https://github.com/wssun/SSLBackdoorMitigation}{https://github.com/wssun/SSLBackdoorMitigation}}, referring to the settings of other datasets to conduct experiments on downstream datasets such as ImageNet and CIFAR-10. For filtering clean data, we implemented META-SIFT following their official open-sourced code Meta-Sift\footnote{\href{https://github.com/ruoxi-jia-group/Meta-Sift}{https://github.com/ruoxi-jia-group/Meta-Sift}}, and for IBD-PSC, SCALE-UP, Spectral, SPECTRE, we referred to the implementation of the code provided by Fight-Poison-With-Poison\footnote{\href{https://github.com/Unispac/Fight-Poison-With-Poison}{https://github.com/Unispac/Fight-Poison-With-Poison}} and made modifications, changing from filtering the poison samples to filtering the clean samples. For post-attack methods, we utilized the implementation available at GitHub\footnote{\href{https://github.com/davda54/sam}{https://github.com/davda54/sam}} for FT-SAM and implemented I-BAU following their official open-sourced code I-BAU\footnote{\href{https://github.com/YiZeng623/I-BAU}{https://github.com/YiZeng623/I-BAU}}.




\section{Supplementary Charts and Tables}
\subsection{Sample Distribution after Confusion Training}
\vspace{-2mm}
\begin{figure}[h]
    \centering
    \subfloat[BadNets]{
        \includegraphics[width=0.21\textwidth]{images/ct_all_loss_badnet.pdf}
        \label{fig:sub1}
    }
    \subfloat[Blended]{
        \includegraphics[width=0.21\textwidth]{images/ct_all_loss_blend.pdf}
        \label{fig:sub2}
    }
\caption{Overall poison and clean sample distribution after Confusion Training: while the low-loss area contains both poisoned and clean samples, the large-loss area is exclusively clean. This plot corresponds to the FT-head in \cref{fig:ct_low_loss}.}
    \label{fig:ct_loss_distribution}
    \vspace{-2mm}
\end{figure}

We plot the loss distribution of training samples after applying CT as an expansion tool in \cref{fig:ct_loss_distribution} under dataset poisoning of BadNet and Blended.

\vspace{-2mm}
\subsection{Performance of Seed Expansion}
We present the results of seed expansion in \cref{tab:expand_samples} under \threattwo. 
% In this experiment, we use the 1\% seed data for expansion, which corresponds to the seed data selection results of a poison ratio of 20\% in \cref{tab:clean_data_sifting}.



\subsection{End-to-End Performance under Dual Threats}
We present T-Core results under the scenario where both \threatone~and \threattwo~exist in \cref{tab:threat4-end2end}.






\begin{table*}[t]
    \centering
    \caption{Number of poisoned samples obtained by seed expansion when expanding till different expansion ratios.
    In each cell, the first number is the number of poisoned samples in the seed data, and the second number is the number of poisoned samples in the added data after seed expansion.
    NTD: \textit{number} of \textit{total} \textit{data}  after seed expansion.
    }
    \adjustbox{center}{
    \resizebox{1\textwidth}{!}{\large
    \setlength{\tabcolsep}{1pt}
    \begin{tabular}{c|cccccccc|cccccccc|cccccccc|cccccccc}
    \toprule
    \multirow{2}{*}{\textbf{Dataset}} & \multicolumn{8}{c|}{\textbf{10\%}} & \multicolumn{8}{c|}{\textbf{20\%}} & \multicolumn{8}{c|}{\textbf{30\%}} & \multicolumn{8}{c}{\textbf{50\%}} \\ \cline{2-33} 
     & \textbf{BadNets} & \textbf{Blended} & \textbf{SIG} & \textbf{WaNet} & \textbf{TaCT} & \textbf{\makecell{~Adap-~\\~Blend~}} & \multicolumn{1}{c|}{\textbf{\makecell{~Adap-~\\~Patch~}}} & \textbf{\begin{tabular}[c]{@{}c@{}}NTD\end{tabular}} & \textbf{BadNets} & \textbf{Blended} & \textbf{SIG} & \textbf{WaNet} & \textbf{TaCT} & \textbf{\makecell{~Adap-~\\~Blend~}} & \multicolumn{1}{c|}{\textbf{\makecell{~Adap-~\\~Patch~}}} & \textbf{\begin{tabular}[c]{@{}c@{}}NTD\end{tabular}} & \textbf{BadNets} & \textbf{Blended} & \textbf{SIG} & \textbf{WaNet} & \textbf{TaCT} & \textbf{\makecell{~Adap-~\\~Blend~}} & \multicolumn{1}{c|}{\textbf{\makecell{~Adap-~\\~Patch~}}} & \textbf{\begin{tabular}[c]{@{}c@{}}NTD\end{tabular}} & \textbf{BadNets} & \textbf{Blended} & \textbf{SIG} & \textbf{WaNet} & \textbf{TaCT} & \textbf{\makecell{~Adap-~\\~Blend~}} & \multicolumn{1}{c|}{\textbf{\makecell{~Adap-~\\~Patch~}}} & \textbf{\begin{tabular}[c]{@{}c@{}}NTD\end{tabular}} \\ \midrule
    \textbf{STL-10} & 0+0 & 0+0 & 0+0 & 0+0 & 0+0 & 0+0 & \multicolumn{1}{c|}{0+0} & 500 & 0+0 & 0+3 & 0+0 & 0+\ 0 & 0+0 & 0+2 & \multicolumn{1}{c|}{0+2} & 1000 & 0+\ 0 & 0+\ 6 & 0+22 & 0+\ 22 & 0+20 & 0+18 & \multicolumn{1}{c|}{0+\ 16} & 1500 & 0+82 & 0+58 & 0+75 & 0+\ 75 & 0+\ 68 & 0+\ 43 & \multicolumn{1}{c|}{0+\ 37} & 2500 \\ \hline
    \textbf{CIFAR-10} & 0+1 & 0+0 & 0+0 & 0+0 & 0+1 & 0+2 & \multicolumn{1}{c|}{0+0} & 5000 & 0+4 & 0+0 & 0+0 & 0+\ 0 & 0+2 & 0+5 & \multicolumn{1}{c|}{0+7} & 10000 & 0+13 & 0+22 & 0+\ 0 & 0+115 & 0+36 & 0+76 & \multicolumn{1}{c|}{0+\ 68} & 15000 & 0+32 & 0+94 & 0+\ 4 & 0+387 & 0+217 & 0+151 & \multicolumn{1}{c|}{0+128} & 25000 \\ \hline
    \textbf{GTSRB} & 0+0 & 0+0 & 0+0 & 0+1 & 0+0 & 0+0 & \multicolumn{1}{c|}{0+0} & 3920 & 0+0 & 0+0 & 0+0 & 0+\ 3 & 0+0 & 0+0 & \multicolumn{1}{c|}{0+1} & 7841 & 0+\ 3 & 0+\ 0 & 0+\ 0 & 0+\ 84 & 0+\ 0 & 0+\ 5 & \multicolumn{1}{c|}{0+\ 17} & 11762 & 0+15 & 0+\ 0 & 0+\ 7 & 0+145 & 0+\ \ 7 & 0+\ \ 5 & \multicolumn{1}{c|}{0+\ 67} & 19604 \\ \hline
    \textbf{SVHN} & 0+0 & 0+0 & 6+1 & 0+5 & 0+1 & 0+3 & \multicolumn{1}{c|}{0+2} & 7325 & 0+1 & 0+3 & 6+5 & 0+22 & 0+5 & 0+5 & \multicolumn{1}{c|}{0+7} & 14651 & 0+\ 6 & 0+22 & 6+23 & 0+\ 67 & 0+20 & 0+22 & \multicolumn{1}{c|}{0+141} & 21977 & 0+14 & 0+89 & 6+77 & 0+245 & 0+\ 32 & 0+\ 65 & \multicolumn{1}{c|}{0+300} & 36628 \\ \hline
    \textbf{ImageNet-10} & 0+0 & 0+0 & 0+0 & 0+2 & 0+0 & 0+0 & \multicolumn{1}{c|}{0+0} & 1006 & 0+0 & 0+0 & 0+0 & 0+\ 7 & 0+0 & 0+0 & \multicolumn{1}{c|}{0+0} & 2012 & 0+\ 0 & 0+\ 0 & 0+\ 7 & 0+\ 13 & 0+\ 0 & 0+\ 4 & \multicolumn{1}{c|}{0+\ 6\ } & 3018 & 0+95 & 0+91 & 0+24 & 0+119 & 0+\ \ 1 & 0+\ 14 & \multicolumn{1}{c|}{0+\ 40} & 5030 \\ \bottomrule
    \end{tabular}
    }
    }
    \label{tab:expand_samples}
\end{table*}



\begin{table*}[t]
    \centering
    \caption{Performance of our end-to-end defense framework under scenarios where both \threatone~and \threattwo~exist. In this setting, transfer learning is subjected to both encoder poisoning and downstream poisoning attacks concurrently, each with a different backdoor trigger. We report the accuracy, the \textit{attack success rate} of the \textit{encoder} poisoning attack (ASR-E), and the \textit{attack success rate} of the \textit{dataset} poisoning attack (ASR-D) for the classifier, both with and without our defense.
    }
    % \begin{center}
    % \tabcolsep=0.05cm
    % \renewcommand{\arraystretch}{1}
    \adjustbox{center}{
    \resizebox{1\textwidth}{!}{
    \setlength{\tabcolsep}{0.5pt}
    \begin{tabular}{c|c|c|c|ccc|ccc|ccc|ccc|ccc|ccc|ccc}
    \toprule
    \rowcolor[HTML]{CCCCCC} 
    \cellcolor[HTML]{CCCCCC}{\color[HTML]{08090C} } & \cellcolor[HTML]{CCCCCC}{\color[HTML]{08090C} } & \cellcolor[HTML]{CCCCCC}{\color[HTML]{08090C} } & \cellcolor[HTML]{CCCCCC}{\color[HTML]{08090C} } & \multicolumn{3}{c|}{\cellcolor[HTML]{CCCCCC}{\color[HTML]{08090C} \textbf{BadNets}}} & \multicolumn{3}{c|}{\cellcolor[HTML]{CCCCCC}{\color[HTML]{08090C} \textbf{Blended}}} & \multicolumn{3}{c|}{\cellcolor[HTML]{CCCCCC}{\color[HTML]{08090C} \textbf{SIG}}} & \multicolumn{3}{c|}{\cellcolor[HTML]{CCCCCC}{\color[HTML]{08090C} \textbf{WaNet}}} & \multicolumn{3}{c|}{\cellcolor[HTML]{CCCCCC}{\color[HTML]{08090C} \textbf{TaCT}}} & \multicolumn{3}{c|}{\cellcolor[HTML]{CCCCCC}{\color[HTML]{08090C} \textbf{Adap-Blend}}} & \multicolumn{3}{c}{\cellcolor[HTML]{CCCCCC}{\color[HTML]{08090C} \textbf{Adap-Patch}}} \\ \cline{5-25} 
    \rowcolor[HTML]{CCCCCC} 
    \multirow{-2}{*}{\cellcolor[HTML]{CCCCCC}{\color[HTML]{08090C} \textbf{\makecell{Encoder\\Poisoning}}}} & \multirow{-2}{*}{\textbf{\makecell{\color[HTML]{08090C} Pre-training \\ Dataset}}} & \multirow{-2}{*}{\textbf{\makecell{\color[HTML]{08090C} Downstream \\ Dataset}}} & \multirow{-2}{*}{\cellcolor[HTML]{CCCCCC}{\color[HTML]{08090C} \textbf{\makecell{Dataset\\Poisoning}}}} & {\color[HTML]{08090C} \textbf{ACC}} & {\color[HTML]{08090C} \textbf{ASR-E}} & {\color[HTML]{08090C} \textbf{ASR-D}} & {\color[HTML]{08090C} \textbf{ACC}} & {\color[HTML]{08090C} \textbf{ASR-E}} & {\color[HTML]{08090C} \textbf{ASR-D}} & {\color[HTML]{08090C} \textbf{ACC}} & {\color[HTML]{08090C} \textbf{ASR-E}} & {\color[HTML]{08090C} \textbf{ASR-D}} & {\color[HTML]{08090C} \textbf{ACC}} & {\color[HTML]{08090C} \textbf{ASR-E}} & {\color[HTML]{08090C} \textbf{ASR-D}} & {\color[HTML]{08090C} \textbf{ACC}} & {\color[HTML]{08090C} \textbf{ASR-E}} & {\color[HTML]{08090C} \textbf{ASR-D}} & {\color[HTML]{08090C} \textbf{ACC}} & {\color[HTML]{08090C} \textbf{ASR-E}} & {\color[HTML]{08090C} \textbf{ASR-D}} & {\color[HTML]{08090C} \textbf{ACC}} & {\color[HTML]{08090C} \textbf{ASR-E}} & {\color[HTML]{08090C} \textbf{ASR-D}} \\ \midrule
     &  &  & No Defense & 76.30 & 99.51 & 91.50 & 76.28 & 99.96 & 60.10 & 76.51 & 99.99 & 59.36 & 76.43 & 99.56 & 4.51 & 75.71 & 99.90 & 62.75 & 76.19 & 96.54 & 10.14 & 76.93 & 99.99 & 1.57 \\
     &  & \multirow{-2}{*}{STL-10} & \cellcolor[HTML]{EFEFEF}Ours & \cellcolor[HTML]{EFEFEF}67.75 & \cellcolor[HTML]{EFEFEF}4.67 & \cellcolor[HTML]{EFEFEF}1.00 & \cellcolor[HTML]{EFEFEF}67.04 & \cellcolor[HTML]{EFEFEF}6.85 & \cellcolor[HTML]{EFEFEF}6.68 & \cellcolor[HTML]{EFEFEF}53.10 & \cellcolor[HTML]{EFEFEF}3.88 & \cellcolor[HTML]{EFEFEF}2.53 & \cellcolor[HTML]{EFEFEF}67.54 & \cellcolor[HTML]{EFEFEF}5.11 & \cellcolor[HTML]{EFEFEF}1.82 & \cellcolor[HTML]{EFEFEF}67.46 & \cellcolor[HTML]{EFEFEF}5.72 & \cellcolor[HTML]{EFEFEF}4.25 & \cellcolor[HTML]{EFEFEF}68.75 & \cellcolor[HTML]{EFEFEF}6.65 & \cellcolor[HTML]{EFEFEF}1.40 & \cellcolor[HTML]{EFEFEF}68.28 & \cellcolor[HTML]{EFEFEF}6.03 & \cellcolor[HTML]{EFEFEF}6.22 \\ \cline{3-25} 
     &  &  & No Defense & 72.60 & 99.24 & 93.75 & 73.22 & 99.77 & 86.36 & 73.16 & 99.15 & 74.81 & 78.17 & 99.94 & 6.09 & 73.86 & 99.20 & 91.73 & 72.98 & 95.95 & 65.60 & 72.22 & 99.69 & 28.43 \\
     &  & \multirow{-2}{*}{GTSRB} & \cellcolor[HTML]{EFEFEF}Ours & \cellcolor[HTML]{EFEFEF}90.54 & \cellcolor[HTML]{EFEFEF}0.01 & \cellcolor[HTML]{EFEFEF}1.38 & \cellcolor[HTML]{EFEFEF}88.27 & \cellcolor[HTML]{EFEFEF}0.31 & \cellcolor[HTML]{EFEFEF}5.05 & \cellcolor[HTML]{EFEFEF}91.69 & \cellcolor[HTML]{EFEFEF}0.00 & \cellcolor[HTML]{EFEFEF}0.98 & \cellcolor[HTML]{EFEFEF}91.88 & \cellcolor[HTML]{EFEFEF}0.04 & \cellcolor[HTML]{EFEFEF}0.66 & \cellcolor[HTML]{EFEFEF}92.60 & \cellcolor[HTML]{EFEFEF}0.80 & \cellcolor[HTML]{EFEFEF}0.00 & \cellcolor[HTML]{EFEFEF}87.79 & \cellcolor[HTML]{EFEFEF}0.00 & \cellcolor[HTML]{EFEFEF}3.30 & \cellcolor[HTML]{EFEFEF}93.90 & \cellcolor[HTML]{EFEFEF}0.27 & \cellcolor[HTML]{EFEFEF}0.29 \\ \cline{3-25} 
     &  &  & No Defense & 68.47 & 98.80 & 99.27 & 67.98 & 98.95 & 98.11 & 68.19 & 98.70 & 96.63 & 67.99 & 98.78 & 11.86 & 68.19 & 98.80 & 94.12 & 68.07 & 98.81 & 90.81 & 68.26 & 97.90 & 71.75 \\
     & \multirow{-6}{*}{CIFAR-10} & \multirow{-2}{*}{SVHN} & \cellcolor[HTML]{EFEFEF}Ours & \cellcolor[HTML]{EFEFEF}92.19 & \cellcolor[HTML]{EFEFEF}4.29 & \cellcolor[HTML]{EFEFEF}3.79 & \cellcolor[HTML]{EFEFEF}92.19 & \cellcolor[HTML]{EFEFEF}4.29 & \cellcolor[HTML]{EFEFEF}0.10 & \cellcolor[HTML]{EFEFEF}92.80 & \cellcolor[HTML]{EFEFEF}4.80 & \cellcolor[HTML]{EFEFEF}0.65 & \cellcolor[HTML]{EFEFEF}90.20 & \cellcolor[HTML]{EFEFEF}7.94 & \cellcolor[HTML]{EFEFEF}2.76 & \cellcolor[HTML]{EFEFEF}91.51 & \cellcolor[HTML]{EFEFEF}2.49 & \cellcolor[HTML]{EFEFEF}0.75 & \cellcolor[HTML]{EFEFEF}90.30 & \cellcolor[HTML]{EFEFEF}4.23 & \cellcolor[HTML]{EFEFEF}0.14 & \cellcolor[HTML]{EFEFEF}92.72 & \cellcolor[HTML]{EFEFEF}4.86 & \cellcolor[HTML]{EFEFEF}0.07 \\ \cline{2-25} 
     &  &  & No Defense & 69.56 & 97.88 & 78.00 & 70.33 & 98.39 & 71.98 & 69.72 & 99.83 & 77.42 & 69.94 & 99.82 & 9.12 & 69.66 & 99.66 & 70.00 & 69.84 & 99.77 & 16.28 & 70.03 & 99.76 & 5.78 \\
     &  & \multirow{-2}{*}{CIFAR-10} & \cellcolor[HTML]{EFEFEF}Ours & \cellcolor[HTML]{EFEFEF}63.27 & \cellcolor[HTML]{EFEFEF}5.76 & \cellcolor[HTML]{EFEFEF}4.76 & \cellcolor[HTML]{EFEFEF}62.73 & \cellcolor[HTML]{EFEFEF}6.28 & \cellcolor[HTML]{EFEFEF}4.97 & \cellcolor[HTML]{EFEFEF}68.42 & \cellcolor[HTML]{EFEFEF}8.29 & \cellcolor[HTML]{EFEFEF}3.64 & \cellcolor[HTML]{EFEFEF}62.63 & \cellcolor[HTML]{EFEFEF}6.61 & \cellcolor[HTML]{EFEFEF}4.47 & \cellcolor[HTML]{EFEFEF}65.47 & \cellcolor[HTML]{EFEFEF}6.36 & \cellcolor[HTML]{EFEFEF}0.00 & \cellcolor[HTML]{EFEFEF}64.38 & \cellcolor[HTML]{EFEFEF}7.71 & \cellcolor[HTML]{EFEFEF}2.03 & \cellcolor[HTML]{EFEFEF}63.05 & \cellcolor[HTML]{EFEFEF}6.08 & \cellcolor[HTML]{EFEFEF}0.13 \\ \cline{3-25} 
     &  &  & No Defense & 70.67 & 97.52 & 83.43 & 69.59 & 98.77 & 82.33 & 70.86 & 99.19 & 74.56 & 69.63 & 99.80 & 4.33 & 68.33 & 98.05 & 81.07 & 68.56 & 99.10 & 54.45 & 69.58 & 98.95 & 12.30 \\
     &  & \multirow{-2}{*}{GTSRB} & \cellcolor[HTML]{EFEFEF}Ours & \cellcolor[HTML]{EFEFEF}85.65 & \cellcolor[HTML]{EFEFEF}0.11 & \cellcolor[HTML]{EFEFEF}5.45 & \cellcolor[HTML]{EFEFEF}86.03 & \cellcolor[HTML]{EFEFEF}0.70 & \cellcolor[HTML]{EFEFEF}0.87 & \cellcolor[HTML]{EFEFEF}85.18 & \cellcolor[HTML]{EFEFEF}1.73 & \cellcolor[HTML]{EFEFEF}0.24 & \cellcolor[HTML]{EFEFEF}85.27 & \cellcolor[HTML]{EFEFEF}0.22 & \cellcolor[HTML]{EFEFEF}4.39 & \cellcolor[HTML]{EFEFEF}86.03 & \cellcolor[HTML]{EFEFEF}0.05 & \cellcolor[HTML]{EFEFEF}1.06 & \cellcolor[HTML]{EFEFEF}85.58 & \cellcolor[HTML]{EFEFEF}1.10 & \cellcolor[HTML]{EFEFEF}5.13 & \cellcolor[HTML]{EFEFEF}87.05 & \cellcolor[HTML]{EFEFEF}1.80 & \cellcolor[HTML]{EFEFEF}1.52 \\ \cline{3-25} 
     &  &  & No Defense & 67.44 & 85.95 & 98.85 & 66.29 & 85.93 & 98.93 & 67.45 & 88.96 & 93.92 & 64.88 & 84.07 & 11.91 & 67.78 & 87.69 & 94.53 & 67.60 & 81.29 & 89.94 & 66.77 & 80.30 & 26.85 \\
    \multirow{-12}{*}{\textbf{BadEncoder}} & \multirow{-6}{*}{STL-10} & \multirow{-2}{*}{SVHN} & \cellcolor[HTML]{EFEFEF}Ours & \cellcolor[HTML]{EFEFEF}83.90 & \cellcolor[HTML]{EFEFEF}4.30 & \cellcolor[HTML]{EFEFEF}10.10 & \cellcolor[HTML]{EFEFEF}86.63 & \cellcolor[HTML]{EFEFEF}3.72 & \cellcolor[HTML]{EFEFEF}5.32 & \cellcolor[HTML]{EFEFEF}85.96 & \cellcolor[HTML]{EFEFEF}9.18 & \cellcolor[HTML]{EFEFEF}2.55 & \cellcolor[HTML]{EFEFEF}88.96 & \cellcolor[HTML]{EFEFEF}5.10 & \cellcolor[HTML]{EFEFEF}1.01 & \cellcolor[HTML]{EFEFEF}86.34 & \cellcolor[HTML]{EFEFEF}3.15 & \cellcolor[HTML]{EFEFEF}0.31 & \cellcolor[HTML]{EFEFEF}86.40 & \cellcolor[HTML]{EFEFEF}4.87 & \cellcolor[HTML]{EFEFEF}2.09 & \cellcolor[HTML]{EFEFEF}86.92 & \cellcolor[HTML]{EFEFEF}6.15 & \cellcolor[HTML]{EFEFEF}4.50 \\ \midrule
     &  &  & No Defense & 71.94 & 99.43 & 75.22 & 71.09 & 98.00 & 53.97 & 72.49 & 93.63 & 35.50 & 72.08 & 90.18 & 10.14 & 71.78 & 97.54 & 49.75 & 71.34 & 99.39 & 11.42 & 71.63 & 98.35 & 1.89 \\
     &  & \multirow{-2}{*}{STL-10} & \cellcolor[HTML]{EFEFEF}Ours & \cellcolor[HTML]{EFEFEF}63.16 & \cellcolor[HTML]{EFEFEF}14.90 & \cellcolor[HTML]{EFEFEF}10.92 & \cellcolor[HTML]{EFEFEF}68.30 & \cellcolor[HTML]{EFEFEF}10.89 & \cellcolor[HTML]{EFEFEF}5.89 & \cellcolor[HTML]{EFEFEF}64.34 & \cellcolor[HTML]{EFEFEF}7.49 & \cellcolor[HTML]{EFEFEF}0.49 & \cellcolor[HTML]{EFEFEF}64.59 & \cellcolor[HTML]{EFEFEF}6.38 & \cellcolor[HTML]{EFEFEF}4.29 & \cellcolor[HTML]{EFEFEF}63.63 & \cellcolor[HTML]{EFEFEF}11.24 & \cellcolor[HTML]{EFEFEF}13.00 & \cellcolor[HTML]{EFEFEF}64.74 & \cellcolor[HTML]{EFEFEF}7.92 & \cellcolor[HTML]{EFEFEF}2.67 & \cellcolor[HTML]{EFEFEF}65.00 & \cellcolor[HTML]{EFEFEF}7.39 & \cellcolor[HTML]{EFEFEF}2.96 \\ \cline{3-25} 
     &  &  & No Defense & 74.35 & 73.36 & 94.19 & 74.57 & 72.99 & 87.63 & 74.95 & 74.70 & 69.57 & 74.48 & 73.02 & 6.58 & 74.67 & 72.91 & 87.07 & 73.95 & 73.01 & 61.30 & 73.76 & 72.97 & 14.79 \\
     &  & \multirow{-2}{*}{GTSRB} & \cellcolor[HTML]{EFEFEF}Ours & \cellcolor[HTML]{EFEFEF}87.98 & \cellcolor[HTML]{EFEFEF}7.05 & \cellcolor[HTML]{EFEFEF}3.16 & \cellcolor[HTML]{EFEFEF}90.17 & \cellcolor[HTML]{EFEFEF}7.23 & \cellcolor[HTML]{EFEFEF}6.66 & \cellcolor[HTML]{EFEFEF}88.16 & \cellcolor[HTML]{EFEFEF}3.18 & \cellcolor[HTML]{EFEFEF}0.74 & \cellcolor[HTML]{EFEFEF}89.14 & \cellcolor[HTML]{EFEFEF}3.61 & \cellcolor[HTML]{EFEFEF}0.47 & \cellcolor[HTML]{EFEFEF}89.93 & \cellcolor[HTML]{EFEFEF}5.82 & \cellcolor[HTML]{EFEFEF}6.82 & \cellcolor[HTML]{EFEFEF}89.14 & \cellcolor[HTML]{EFEFEF}5.05 & \cellcolor[HTML]{EFEFEF}7.63 & \cellcolor[HTML]{EFEFEF}89.87 & \cellcolor[HTML]{EFEFEF}3.10 & \cellcolor[HTML]{EFEFEF}1.85 \\ \cline{3-25} 
     &  &  & No Defense & 71.35 & 75.53 & 99.45 & 71.37 & 75.74 & 97.60 & 71.21 & 75.81 & 94.45 & 71.04 & 76.95 & 11.60 & 71.31 & 72.91 & 96.35 & 71.26 & 77.03 & 85.17 & 71.09 & 76.30 & 51.23 \\
     & \multirow{-6}{*}{CIFAR-10} & \multirow{-2}{*}{SVHN} & \cellcolor[HTML]{EFEFEF}Ours & \cellcolor[HTML]{EFEFEF}89.54 & \cellcolor[HTML]{EFEFEF}9.64 & \cellcolor[HTML]{EFEFEF}6.78 & \cellcolor[HTML]{EFEFEF}88.73 & \cellcolor[HTML]{EFEFEF}6.92 & \cellcolor[HTML]{EFEFEF}4.90 & \cellcolor[HTML]{EFEFEF}89.02 & \cellcolor[HTML]{EFEFEF}9.88 & \cellcolor[HTML]{EFEFEF}4.32 & \cellcolor[HTML]{EFEFEF}87.19 & \cellcolor[HTML]{EFEFEF}6.66 & \cellcolor[HTML]{EFEFEF}3.66 & \cellcolor[HTML]{EFEFEF}92.34 & \cellcolor[HTML]{EFEFEF}3.60 & \cellcolor[HTML]{EFEFEF}2.77 & \cellcolor[HTML]{EFEFEF}89.20 & \cellcolor[HTML]{EFEFEF}5.10 & \cellcolor[HTML]{EFEFEF}1.01 & \cellcolor[HTML]{EFEFEF}89.70 & \cellcolor[HTML]{EFEFEF}5.04 & \cellcolor[HTML]{EFEFEF}2.97 \\ \cline{2-25} 
     &  &  & No Defense & 70.26 & 78.54 & 74.24 & 70.71 & 77.58 & 74.19 & 70.83 & 79.10 & 69.62 & 70.87 & 78.66 & 9.27 & 70.62 & 78.55 & 69.00 & 70.81 & 78.63 & 14.13 & 71.15 & 78.63 & 4.93 \\
     &  & \multirow{-2}{*}{CIFAR-10} & \cellcolor[HTML]{EFEFEF}Ours & \cellcolor[HTML]{EFEFEF}64.74 & \cellcolor[HTML]{EFEFEF}6.87 & \cellcolor[HTML]{EFEFEF}7.43 & \cellcolor[HTML]{EFEFEF}63.46 & \cellcolor[HTML]{EFEFEF}7.53 & \cellcolor[HTML]{EFEFEF}7.69 & \cellcolor[HTML]{EFEFEF}67.31 & \cellcolor[HTML]{EFEFEF}4.94 & \cellcolor[HTML]{EFEFEF}1.91 & \cellcolor[HTML]{EFEFEF}66.18 & \cellcolor[HTML]{EFEFEF}4.02 & \cellcolor[HTML]{EFEFEF}1.73 & \cellcolor[HTML]{EFEFEF}66.28 & \cellcolor[HTML]{EFEFEF}5.49 & \cellcolor[HTML]{EFEFEF}0.10 & \cellcolor[HTML]{EFEFEF}62.63 & \cellcolor[HTML]{EFEFEF}4.96 & \cellcolor[HTML]{EFEFEF}3.40 & \cellcolor[HTML]{EFEFEF}63.56 & \cellcolor[HTML]{EFEFEF}3.31 & \cellcolor[HTML]{EFEFEF}6.31 \\ \cline{3-25} 
     &  &  & No Defense & 63.40 & 78.25 & 90.50 & 63.71 & 84.92 & 88.70 & 64.29 & 85.40 & 74.55 & 63.99 & 78.12 & 6.09 & 63.47 & 86.80 & 78.54 & 61.18 & 80.32 & 67.40 & 62.00 & 79.83 & 18.46 \\
     &  & \multirow{-2}{*}{GTSRB} & \cellcolor[HTML]{EFEFEF}Ours & \cellcolor[HTML]{EFEFEF}86.10 & \cellcolor[HTML]{EFEFEF}0.21 & \cellcolor[HTML]{EFEFEF}3.94 & \cellcolor[HTML]{EFEFEF}87.08 & \cellcolor[HTML]{EFEFEF}1.42 & \cellcolor[HTML]{EFEFEF}5.85 & \cellcolor[HTML]{EFEFEF}86.44 & \cellcolor[HTML]{EFEFEF}2.82 & \cellcolor[HTML]{EFEFEF}0.03 & \cellcolor[HTML]{EFEFEF}84.47 & \cellcolor[HTML]{EFEFEF}1.00 & \cellcolor[HTML]{EFEFEF}3.18 & \cellcolor[HTML]{EFEFEF}82.18 & \cellcolor[HTML]{EFEFEF}0.25 & \cellcolor[HTML]{EFEFEF}5.45 & \cellcolor[HTML]{EFEFEF}81.90 & \cellcolor[HTML]{EFEFEF}1.61 & \cellcolor[HTML]{EFEFEF}2.95 & \cellcolor[HTML]{EFEFEF}81.32 & \cellcolor[HTML]{EFEFEF}0.62 & \cellcolor[HTML]{EFEFEF}7.58 \\ \cline{3-25} 
     &  &  & No Defense & 59.12 & 94.66 & 96.56 & 59.77 & 97.48 & 97.43 & 58.03 & 92.94 & 91.53 & 59.77 & 95.08 & 15.17 & 59.47 & 97.46 & 92.33 & 60.02 & 98.69 & 84.58 & 59.74 & 96.81 & 16.52 \\
    \multirow{-12}{*}{\textbf{DRUPE}} & \multirow{-6}{*}{STL-10} & \multirow{-2}{*}{SVHN} & \cellcolor[HTML]{EFEFEF}Ours & \cellcolor[HTML]{EFEFEF}82.13 & \cellcolor[HTML]{EFEFEF}5.95 & \cellcolor[HTML]{EFEFEF}6.25 & \cellcolor[HTML]{EFEFEF}83.22 & \cellcolor[HTML]{EFEFEF}4.03 & \cellcolor[HTML]{EFEFEF}4.56 & \cellcolor[HTML]{EFEFEF}83.75 & \cellcolor[HTML]{EFEFEF}9.64 & \cellcolor[HTML]{EFEFEF}2.77 & \cellcolor[HTML]{EFEFEF}82.76 & \cellcolor[HTML]{EFEFEF}2.45 & \cellcolor[HTML]{EFEFEF}3.59 & \cellcolor[HTML]{EFEFEF}83.85 & \cellcolor[HTML]{EFEFEF}2.93 & \cellcolor[HTML]{EFEFEF}0.98 & \cellcolor[HTML]{EFEFEF}81.13 & \cellcolor[HTML]{EFEFEF}9.01 & \cellcolor[HTML]{EFEFEF}5.10 & \cellcolor[HTML]{EFEFEF}83.17 & \cellcolor[HTML]{EFEFEF}3.05 & \cellcolor[HTML]{EFEFEF}1.65 \\ \midrule
     &  &  & No Defense & 51.80 & 9.97 & 56.39 & 53.20 & 10.15 & 17.67 & 53.14 & 8.99 & 18.96 & 53.43 & 10.19 & 5.75 & 52.06 & 10.83 & 40.25 & 53.28 & 8.79 & 4.99 & 52.88 & 8.65 & 4.64 \\
     & \multirow{-2}{*}{STL-10} & \multirow{-2}{*}{STL-10} & \cellcolor[HTML]{EFEFEF}Ours & \cellcolor[HTML]{EFEFEF}48.81 & \cellcolor[HTML]{EFEFEF}1.79 & \cellcolor[HTML]{EFEFEF}1.21 & \cellcolor[HTML]{EFEFEF}49.80 & \cellcolor[HTML]{EFEFEF}2.23 & \cellcolor[HTML]{EFEFEF}2.51 & \cellcolor[HTML]{EFEFEF}45.56 & \cellcolor[HTML]{EFEFEF}3.57 & \cellcolor[HTML]{EFEFEF}0.99 & \cellcolor[HTML]{EFEFEF}49.68 & \cellcolor[HTML]{EFEFEF}0.24 & \cellcolor[HTML]{EFEFEF}2.44 & \cellcolor[HTML]{EFEFEF}50.43 & \cellcolor[HTML]{EFEFEF}2.58 & \cellcolor[HTML]{EFEFEF}3.51 & \cellcolor[HTML]{EFEFEF}49.63 & \cellcolor[HTML]{EFEFEF}2.44 & \cellcolor[HTML]{EFEFEF}5.93 & \cellcolor[HTML]{EFEFEF}48.44 & \cellcolor[HTML]{EFEFEF}1.03 & \cellcolor[HTML]{EFEFEF}1.96 \\ \cline{2-25} 
     &  &  & No Defense & 75.33 & 48.93 & 93.29 & 75.22 & 44.92 & 50.59 & 76.19 & 38.54 & 52.56 & 74.31 & 41.14 & 13.98 & 75.80 & 48.87 & 84.00 & 75.08 & 49.41 & 16.93 & 75.93 & 46.74 & 14.90 \\
     & \multirow{-2}{*}{CIFAR-10} & \multirow{-2}{*}{CIFAR-10} & \cellcolor[HTML]{EFEFEF}Ours & \cellcolor[HTML]{EFEFEF}61.78 & \cellcolor[HTML]{EFEFEF}0.94 & \cellcolor[HTML]{EFEFEF}0.10 & \cellcolor[HTML]{EFEFEF}62.72 & \cellcolor[HTML]{EFEFEF}2.87 & \cellcolor[HTML]{EFEFEF}6.88 & \cellcolor[HTML]{EFEFEF}61.94 & \cellcolor[HTML]{EFEFEF}0.59 & \cellcolor[HTML]{EFEFEF}0.00 & \cellcolor[HTML]{EFEFEF}62.32 & \cellcolor[HTML]{EFEFEF}3.60 & \cellcolor[HTML]{EFEFEF}3.44 & \cellcolor[HTML]{EFEFEF}62.79 & \cellcolor[HTML]{EFEFEF}0.57 & \cellcolor[HTML]{EFEFEF}0.70 & \cellcolor[HTML]{EFEFEF}63.51 & \cellcolor[HTML]{EFEFEF}8.78 & \cellcolor[HTML]{EFEFEF}8.84 & \cellcolor[HTML]{EFEFEF}58.80 & \cellcolor[HTML]{EFEFEF}0.63 & \cellcolor[HTML]{EFEFEF}6.72 \\ \cline{2-25} 
     &  &  & No Defense & 64.68 & 4.60 & 73.81 & 67.16 & 3.05 & 69.37 & 65.83 & 4.96 & 60.30 & 66.00 & 3.76 & 4.67 & 65.86 & 5.82 & 62.40 & 66.94 & 0.94 & 52.71 & 65.13 & 4.84 & 21.36 \\
    \multirow{-6}{*}{\textbf{CTRL}} & \multirow{-2}{*}{GTSRB} & \multirow{-2}{*}{GTSRB} & \cellcolor[HTML]{EFEFEF}Ours & \cellcolor[HTML]{EFEFEF}85.30 & \cellcolor[HTML]{EFEFEF}0.09 & \cellcolor[HTML]{EFEFEF}2.79 & \cellcolor[HTML]{EFEFEF}88.28 & \cellcolor[HTML]{EFEFEF}0.19 & \cellcolor[HTML]{EFEFEF}0.14 & \cellcolor[HTML]{EFEFEF}87.05 & \cellcolor[HTML]{EFEFEF}0.00 & \cellcolor[HTML]{EFEFEF}0.07 & \cellcolor[HTML]{EFEFEF}87.82 & \cellcolor[HTML]{EFEFEF}0.08 & \cellcolor[HTML]{EFEFEF}0.34 & \cellcolor[HTML]{EFEFEF}88.37 & \cellcolor[HTML]{EFEFEF}0.15 & \cellcolor[HTML]{EFEFEF}0.40 & \cellcolor[HTML]{EFEFEF}88.13 & \cellcolor[HTML]{EFEFEF}1.77 & \cellcolor[HTML]{EFEFEF}4.97 & \cellcolor[HTML]{EFEFEF}87.73 & \cellcolor[HTML]{EFEFEF}0.11 & \cellcolor[HTML]{EFEFEF}0.03 \\ \midrule
     &  &  & No Defense & 84.47 & 19.15 & 84.79 & 83.88 & 24.97 & 32.85 & 82.85 & 45.88 & 60.00 & 81.18 & 24.61 & 2.48 & 83.12 & 40.18 & 93.00 & 82.47 & 26.36 & 26.42 & 82.94 & 33.70 & 2.24 \\
    \multirow{-2}{*}{\textbf{SSLBackdoor}} & \multirow{-2}{*}{ImageNet} & \multirow{-2}{*}{ImageNet-10} & \cellcolor[HTML]{EFEFEF}Ours & \cellcolor[HTML]{EFEFEF}80.65 & \cellcolor[HTML]{EFEFEF}2.61 & \cellcolor[HTML]{EFEFEF}3.15 & \cellcolor[HTML]{EFEFEF}80.82 & \cellcolor[HTML]{EFEFEF}1.21 & \cellcolor[HTML]{EFEFEF}6.55 & \cellcolor[HTML]{EFEFEF}79.94 & \cellcolor[HTML]{EFEFEF}3.21 & \cellcolor[HTML]{EFEFEF}4.97 & \cellcolor[HTML]{EFEFEF}78.00 & \cellcolor[HTML]{EFEFEF}3.21 & \cellcolor[HTML]{EFEFEF}2.24 & \cellcolor[HTML]{EFEFEF}83.47 & \cellcolor[HTML]{EFEFEF}1.88 & \cellcolor[HTML]{EFEFEF}3.21 & \cellcolor[HTML]{EFEFEF}83.18 & \cellcolor[HTML]{EFEFEF}0.67 & \cellcolor[HTML]{EFEFEF}3.82 & \cellcolor[HTML]{EFEFEF}83.47 & \cellcolor[HTML]{EFEFEF}1.82 & \cellcolor[HTML]{EFEFEF}2.61 \\ \midrule
     &  &  & No Defense & 84.41 & 34.91 & 82.73 & 83.76 & 57.45 & 26.73 & 82.53 & 54.18 & 61.82 & 81.41 & 44.06 & 3.94 & 83.76 & 60.12 & 91.00 & 80.06 & 53.09 & 15.03 & 83.47 & 57.27 & 3.45 \\
    \multirow{-2}{*}{\textbf{CorruptEncoder}} & \multirow{-2}{*}{ImageNet} & \multirow{-2}{*}{ImageNet-10} & \cellcolor[HTML]{EFEFEF}Ours & \cellcolor[HTML]{EFEFEF}82.35 & \cellcolor[HTML]{EFEFEF}1.33 & \cellcolor[HTML]{EFEFEF}4.55 & \cellcolor[HTML]{EFEFEF}82.35 & \cellcolor[HTML]{EFEFEF}2.00 & \cellcolor[HTML]{EFEFEF}4.61 & \cellcolor[HTML]{EFEFEF}82.06 & \cellcolor[HTML]{EFEFEF}1.33 & \cellcolor[HTML]{EFEFEF}5.88 & \cellcolor[HTML]{EFEFEF}80.00 & \cellcolor[HTML]{EFEFEF}1.58 & \cellcolor[HTML]{EFEFEF}3.15 & \cellcolor[HTML]{EFEFEF}81.65 & \cellcolor[HTML]{EFEFEF}1.21 & \cellcolor[HTML]{EFEFEF}6.50 & \cellcolor[HTML]{EFEFEF}82.53 & \cellcolor[HTML]{EFEFEF}0.97 & \cellcolor[HTML]{EFEFEF}6.36 & \cellcolor[HTML]{EFEFEF}84.06 & \cellcolor[HTML]{EFEFEF}1.82 & \cellcolor[HTML]{EFEFEF}1.76 \\ 
      
    
    \bottomrule
    \end{tabular}
    }
    }
    \label{tab:threat4-end2end}
    \vspace{-4mm}
\end{table*}


% \begin{table}[t]
%       \centering
%       \caption{Peformance of our entire end-to-end defense framework under \threatone.
%       In this setting, transfer learning is subjected to encoder poisoning alone. 
%       We report the accuracy and the attack success rate both with and without our defense.
%             }
%             \adjustbox{width=0.45\textwidth, center}{\large
%             \setlength{\tabcolsep}{0.5pt}
%             \begin{tabular}{c|c|c|c|cc|c|c|c|c|cc}
%                 \toprule
%                 \rowcolor[HTML]{CCCCCC} 
%                 { \textbf{\color[HTML]{08090C}\makecell{Encoder\ \ \\Poisoning\ \ \ }}}& {\textbf{\makecell{\color[HTML]{08090C} Pre-training \\ Dataset}}} & {\textbf{\makecell{\color[HTML]{08090C} Downstream \\ Dataset}}} & {\color[HTML]{08090C} \textbf{Methods}} & {\color[HTML]{08090C} \textbf{ACC$\uparrow$}} & {\color[HTML]{08090C} \textbf{ASR$\downarrow$}} & {\textbf{\color[HTML]{08090C}\makecell{\ \ \ \ Encoder\ \ \ \ \\\ \ \ \ \ \ Poisoning\ \ \ \ \ \   }}} & {\textbf{\makecell{\color[HTML]{08090C} Pre-training \\ Dataset}}} & {\textbf{\makecell{\color[HTML]{08090C} Downstream \\ Dataset}}} & {\color[HTML]{08090C} \textbf{Methods}} & {\color[HTML]{08090C} \textbf{ACC$\uparrow$}} & {\color[HTML]{08090C} \textbf{ASR$\downarrow$}} \\ \midrule
%                 &  &  & No Defense & 76.58 & 98.51 &  &  &  & No Defense & 71.85 & 97.72 \\
%                 &  & \multirow{-2}{*}{STL-10} & \cellcolor[HTML]{EFEFEF}Ours & \cellcolor[HTML]{EFEFEF}55.23 & \cellcolor[HTML]{EFEFEF}4.29 &  &  & \multirow{-2}{*}{STL-10} & \cellcolor[HTML]{EFEFEF}Ours & \cellcolor[HTML]{EFEFEF}54.54 & \cellcolor[HTML]{EFEFEF}6.28 \\ \cline{3-6} \cline{9-12} 
%                 &  &  & No Defense & 80.77 & 99.63 &  &  &  & No Defense & 76.39 & 98.10 \\
%                 &  & \multirow{-2}{*}{GTSRB} & \cellcolor[HTML]{EFEFEF}Ours & \cellcolor[HTML]{EFEFEF}90.86 & \cellcolor[HTML]{EFEFEF}3.90 &  &  & \multirow{-2}{*}{GTSRB} & \cellcolor[HTML]{EFEFEF}Ours & \cellcolor[HTML]{EFEFEF}93.28 & \cellcolor[HTML]{EFEFEF}4.50 \\ \cline{3-6} \cline{9-12} 
%                 &  &  & No Defense & 65.35 & 97.56 &  &  &  & No Defense & 72.99 & 92.71 \\
%                 & \multirow{-6}{*}{CIFAR-10} & \multirow{-2}{*}{SVHN} & \cellcolor[HTML]{EFEFEF}Ours & \cellcolor[HTML]{EFEFEF}85.93 & \cellcolor[HTML]{EFEFEF}3.76 &  & \multirow{-6}{*}{CIFAR-10} & \multirow{-2}{*}{SVHN} & \cellcolor[HTML]{EFEFEF}Ours & \cellcolor[HTML]{EFEFEF}87.27 & \cellcolor[HTML]{EFEFEF}6.47 \\ \cline{2-6} \cline{8-12} 
%                 &  &  & No Defense & 70.57 & 98.93 &  &  &  & No Defense & 71.14 & 80.49 \\
%                 &  & \multirow{-2}{*}{CIFAR-10} & \cellcolor[HTML]{EFEFEF}Ours & \cellcolor[HTML]{EFEFEF}60.65 & \cellcolor[HTML]{EFEFEF}5.22 &  &  & \multirow{-2}{*}{CIFAR-10} & \cellcolor[HTML]{EFEFEF}Ours & \cellcolor[HTML]{EFEFEF}63.93 & \cellcolor[HTML]{EFEFEF}1.61 \\ \cline{3-6} \cline{9-12} 
%                 &  &  & No Defense & 70.83 & 98.99 &  &  &  & No Defense & 65.11 & 85.03 \\
%                 &  & \multirow{-2}{*}{GTSRB} & \cellcolor[HTML]{EFEFEF}Ours & \cellcolor[HTML]{EFEFEF}87.08 & \cellcolor[HTML]{EFEFEF}4.93 &  &  & \multirow{-2}{*}{GTSRB} & \cellcolor[HTML]{EFEFEF}Ours & \cellcolor[HTML]{EFEFEF}84.51 & \cellcolor[HTML]{EFEFEF}3.97 \\ \cline{3-6} \cline{9-12} 
%                 &  &  & No Defense & 64.89 & 98.98 &  &  &  & No Defense & 58.43 & 96.28 \\
%                 \multirow{-12}{*}{\textbf{BadEncoder}} & \multirow{-6}{*}{STL-10} & \multirow{-2}{*}{SVHN} & \cellcolor[HTML]{EFEFEF}Ours & \cellcolor[HTML]{EFEFEF}86.76 & \cellcolor[HTML]{EFEFEF}6.09 & \multirow{-12}{*}{\textbf{DRUPE}} & \multirow{-6}{*}{STL-10} & \multirow{-2}{*}{SVHN} & \cellcolor[HTML]{EFEFEF}Ours & \cellcolor[HTML]{EFEFEF}87.37 & \cellcolor[HTML]{EFEFEF}5.58 \\ \midrule
%                 &  &  & No Defense & 52.15 & 9.88 &  &  &  & No Defense & 82.85 & 36.48 \\
%                 & \multirow{-2}{*}{STL-10} & \multirow{-2}{*}{STL-10} & \cellcolor[HTML]{EFEFEF}Ours & \cellcolor[HTML]{EFEFEF}48.01 & \cellcolor[HTML]{EFEFEF}0.18 & \multirow{-2}{*}{\textbf{SSLBackdoor}} & \multirow{-2}{*}{ImageNet} & \multirow{-2}{*}{ImageNet-10} & \cellcolor[HTML]{EFEFEF}Ours & \cellcolor[HTML]{EFEFEF}72.35 & \cellcolor[HTML]{EFEFEF}0.42 \\ \cline{2-12} 
%                 &  &  & No Defense & 75.31 & 44.90 &  &  &  & No Defense & 82.35 & 58.46 \\
%                 & \multirow{-2}{*}{CIFAR-10} & \multirow{-2}{*}{CIFAR-10} & \cellcolor[HTML]{EFEFEF}Ours & \cellcolor[HTML]{EFEFEF}56.66 & \cellcolor[HTML]{EFEFEF}3.07 & \multirow{-2}{*}{\textbf{CorruptEncoder}} & \multirow{-2}{*}{ImageNet} & \multirow{-2}{*}{ImageNet-10} & \cellcolor[HTML]{EFEFEF}Ours & \cellcolor[HTML]{EFEFEF}72.82 & \cellcolor[HTML]{EFEFEF}1.03 \\ \cline{2-12} 
%                 &  &  & No Defense & 66.78 & 6.54 &  &  &  & No Defense & \cellcolor[HTML]{EFEFEF}85.94 & \cellcolor[HTML]{EFEFEF}78.06 \\
%                 \multirow{-6}{*}{\textbf{CTRL}} & \multirow{-2}{*}{GTSRB} & \multirow{-2}{*}{GTSRB} & \cellcolor[HTML]{EFEFEF}Ours & \cellcolor[HTML]{EFEFEF}82.42 & \cellcolor[HTML]{EFEFEF}0.87 & \multirow{-2}{*}{\textbf{CorruptEncoder+}} & \multirow{-2}{*}{ImageNet} & \multirow{-2}{*}{ImageNet-10} & \cellcolor[HTML]{EFEFEF}Ours & \cellcolor[HTML]{EFEFEF}69.00 & \cellcolor[HTML]{EFEFEF}1.58 \\ \bottomrule
%             \end{tabular}
% }
% \label{tab:threat1-end2end}
% \end{table}







% \begin{table}[t]
%     \centering
%     \caption{Performance of our entire end-to-end defense framework under \threatthree.
% In this setting, transfer learning is subjected to encoder poisoning and downstream dataset poisoning with the same backdoor trigger of the poisoned encoder. 
% We report the accuracy and the attack success rate both with and without our defense.
%       }
%       \adjustbox{width=0.45\textwidth, center}{\large
%       \setlength{\tabcolsep}{0.5pt}
%       \begin{tabular}{c|c|c|c|cc|c|c|c|c|cc}
%       \toprule
%       \rowcolor[HTML]{CCCCCC} 
%       { \textbf{\color[HTML]{08090C}\makecell{Encoder\ \ \\Poisoning\ \ \ }}}& {\textbf{\makecell{\color[HTML]{08090C} Pre-training \\ Dataset}}} & {\textbf{\makecell{\color[HTML]{08090C} Downstream \\ Dataset}}} & {\color[HTML]{08090C} \textbf{Methods}} & {\color[HTML]{08090C} \textbf{ACC$\uparrow$}} & {\color[HTML]{08090C} \textbf{ASR$\downarrow$}} & {\textbf{\color[HTML]{08090C}\makecell{\ \ \ \ Encoder\ \ \ \ \\\ \ \ \ \ \ Poisoning\ \ \ \ \ \   }}} & {\textbf{\makecell{\color[HTML]{08090C} Pre-training \\ Dataset}}} & {\textbf{\makecell{\color[HTML]{08090C} Downstream \\ Dataset}}} & {\color[HTML]{08090C} \textbf{Methods}} & {\color[HTML]{08090C} \textbf{ACC$\uparrow$}} & {\color[HTML]{08090C} \textbf{ASR$\downarrow$}} \\ \midrule
%       &  &  & No Defense & 76.79 & 100.00 &  &  &  & No Defense & 72.39 & 99.94 \\
%       &  & \multirow{-2}{*}{STL-10} & \cellcolor[HTML]{EFEFEF}Ours & \cellcolor[HTML]{EFEFEF}66.24 & \cellcolor[HTML]{EFEFEF}1.40 &  &  & \multirow{-2}{*}{STL-10} & \cellcolor[HTML]{EFEFEF}Ours & \cellcolor[HTML]{EFEFEF}66.38 & \cellcolor[HTML]{EFEFEF}5.19 \\ \cline{3-6} \cline{9-12} 
%       &  &  & No Defense & 78.45 & 99.97 &  &  &  & No Defense & 75.22 & 99.20 \\
%       &  & \multirow{-2}{*}{GTSRB} & \cellcolor[HTML]{EFEFEF}Ours & \cellcolor[HTML]{EFEFEF}91.92 & \cellcolor[HTML]{EFEFEF}0.01 &  &  & \multirow{-2}{*}{GTSRB} & \cellcolor[HTML]{EFEFEF}Ours & \cellcolor[HTML]{EFEFEF}90.65 & \cellcolor[HTML]{EFEFEF}3.73 \\ \cline{3-6} \cline{9-12} 
%       &  &  & No Defense & 67.93 & 99.44 &  &  &  & No Defense & 71.34 & 99.87 \\
%       & \multirow{-6}{*}{CIFAR-10} & \multirow{-2}{*}{SVHN} & \cellcolor[HTML]{EFEFEF}Ours & \cellcolor[HTML]{EFEFEF}92.52 & \cellcolor[HTML]{EFEFEF}0.65 &  & \multirow{-6}{*}{CIFAR-10} & \multirow{-2}{*}{SVHN} & \cellcolor[HTML]{EFEFEF}Ours & \cellcolor[HTML]{EFEFEF}89.57 & \cellcolor[HTML]{EFEFEF}3.60 \\ \cline{2-6} \cline{8-12} 
%       &  &  & No Defense & 69.66 & 99.96 &  &  &  & No Defense & 71.21 & 99.66 \\
%       &  & \multirow{-2}{*}{CIFAR-10} & \cellcolor[HTML]{EFEFEF}Ours & \cellcolor[HTML]{EFEFEF}62.90 & \cellcolor[HTML]{EFEFEF}6.80 &  &  & \multirow{-2}{*}{CIFAR-10} & \cellcolor[HTML]{EFEFEF}Ours & \cellcolor[HTML]{EFEFEF}63.07 & \cellcolor[HTML]{EFEFEF}5.70 \\ \cline{3-6} \cline{9-12} 
%       &  &  & No Defense & 66.67 & 99.83 &  &  &  & No Defense & 64.90 & 99.18 \\
%       &  & \multirow{-2}{*}{GTSRB} & \cellcolor[HTML]{EFEFEF}Ours & \cellcolor[HTML]{EFEFEF}90.43 & \cellcolor[HTML]{EFEFEF}0.76 &  &  & \multirow{-2}{*}{GTSRB} & \cellcolor[HTML]{EFEFEF}Ours & \cellcolor[HTML]{EFEFEF}85.82 & \cellcolor[HTML]{EFEFEF}0.86 \\ \cline{3-6} \cline{9-12} 
%       &  &  & No Defense & 63.55 & 99.57 &  &  &  & No Defense & 58.35 & 99.66 \\
%       \multirow{-12}{*}{\textbf{BadEncoder}} & \multirow{-6}{*}{STL-10} & \multirow{-2}{*}{SVHN} & \cellcolor[HTML]{EFEFEF}Ours & \cellcolor[HTML]{EFEFEF}87.34 & \cellcolor[HTML]{EFEFEF}0.54 & \multirow{-12}{*}{\textbf{DRUPE}} & \multirow{-6}{*}{STL-10} & \multirow{-2}{*}{SVHN} & \cellcolor[HTML]{EFEFEF}Ours & \cellcolor[HTML]{EFEFEF}83.91 & \cellcolor[HTML]{EFEFEF}0.37 \\ \midrule
%       &  &  & No Defense & 53.08 & 9.81 &  &  &  & No Defense & 83.29 & 87.94 \\
%       & \multirow{-2}{*}{STL-10} & \multirow{-2}{*}{STL-10} & \cellcolor[HTML]{EFEFEF}Ours & \cellcolor[HTML]{EFEFEF}48.56 & \cellcolor[HTML]{EFEFEF}1.41 & \multirow{-2}{*}{\textbf{SSLBackdoor}} & \multirow{-2}{*}{ImageNet} & \multirow{-2}{*}{ImageNet-10} & \cellcolor[HTML]{EFEFEF}Ours & \cellcolor[HTML]{EFEFEF}81.35 & \cellcolor[HTML]{EFEFEF}1.76 \\ \cline{2-12} 
%       &  &  & No Defense & 75.63 & 53.56 &  &  &  & No Defense & 82.47 & 92.12 \\
%       & \multirow{-2}{*}{CIFAR-10} & \multirow{-2}{*}{CIFAR-10} & \cellcolor[HTML]{EFEFEF}Ours & \cellcolor[HTML]{EFEFEF}59.35 & \cellcolor[HTML]{EFEFEF}3.72 & \multirow{-2}{*}{\textbf{CorruptEncoder}} & \multirow{-2}{*}{ImageNet} & \multirow{-2}{*}{ImageNet-10} & \cellcolor[HTML]{EFEFEF}Ours & \cellcolor[HTML]{EFEFEF}81.47 & \cellcolor[HTML]{EFEFEF}4.79 \\ \cline{2-12} 
%       &  &  & No Defense & 64.29 & 26.11 &  &  &  & No Defense & 84.29 & 97.52  \\
%       \multirow{-6}{*}{\textbf{CTRL}} & \multirow{-2}{*}{GTSRB} & \multirow{-2}{*}{GTSRB} & \cellcolor[HTML]{EFEFEF}Ours & \cellcolor[HTML]{EFEFEF}88.11 & \cellcolor[HTML]{EFEFEF}1.91 & \multirow{-2}{*}{\textbf{CorruptEncoder+}} & \multirow{-2}{*}{ImageNet} & \multirow{-2}{*}{ImageNet-10} & \cellcolor[HTML]{EFEFEF}Ours & \cellcolor[HTML]{EFEFEF}81.47 & \cellcolor[HTML]{EFEFEF}5.58 \\ \bottomrule
%       \end{tabular}
%         \label{tab:threat3-end2end}
%       }
% \end{table}



\clearpage

% \begin{table}[]
%     \centering
%     \caption{
%     Finetune all after distillation
%     }
%     \adjustbox{center}{
%     \resizebox{0.47\textwidth}{!}{\large
%     \setlength{\tabcolsep}{0.5pt}
% \begin{tabular}{c|c|c|cc|cc}
% \toprule
% \multirow{2}{*}{\makecell{Encoder\\Poisoning}} & \multirow{2}{*}{\makecell{Pretraining\\Dataset}} & \multirow{2}{*}{\makecell{Downstream\\Dataset}} & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}SSL-\\Distillation$_\textrm{up}$\end{tabular}} & \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}SSL-\\Distillation$_\textrm{down}$\end{tabular}} \\ \cline{4-7} 
%  &  &  & ASR$\downarrow$ & ACC$\uparrow$ & ASR$\downarrow$ & ACC$\uparrow$ \\ \hline
% \multirow{6}{*}{BadEncoder} & \multirow{3}{*}{CIFAR-10} & STL-10 & 4.64 & 69.58 & 6.22 & 41.43 \\ \cline{3-7} 
%  &  & GTSRB & 0.23 & 95.49 & 0.77 & 95.78 \\ \cline{3-7} 
%  &  & SVHN & 9.45 & 95.14 & 6.54 & 95.11 \\ \cline{2-7} 
%  & \multirow{3}{*}{STL-10} & CIFAR-10 & 20.93 & 77.14 & 12.39 & 78.53 \\ \cline{3-7} 
%  &  & GTSRB & 0.12 & 94.89 & 0.01 & 95.84 \\ \cline{3-7} 
%  &  & SVHN & 4.43 & 92.96 & 2.89 & 93.32 \\ \hline
% \multirow{6}{*}{DRUPE} & \multirow{3}{*}{CIFAR-10} & STL-10 & 13.89 & 66.20 & 7.60 & 41.58 \\ \cline{3-7} 
%  &  & GTSRB & 0.02 & 95.52 & 0.01 & 97.56 \\ \cline{3-7} 
%  &  & SVHN & 4.43 & 94.62 & 15.44 & 94.50 \\ \cline{2-7} 
%  & \multirow{3}{*}{STL-10} & CIFAR-10 & 19.66 & 76.86 & 18.80 & 79.27 \\ \cline{3-7} 
%  &  & GTSRB & 0.08 & 94.83 & 0.10 & 95.47 \\ \cline{3-7} 
%  &  & SVHN & 5.76 & 93.23 & 7.04 & 93.58 \\ \hline
% \multirow{3}{*}{CTRL} & STL-10 & STL-10 & - & - & 1.07 & 59.19 \\ \cline{2-7} 
%  & CIFAR-10 & CIFAR-10 & - & - & 5.03 & 70.06 \\ \cline{2-7} 
%  & GTSRB & GTSRB & - & - & 0.88 & 90.27 \\ \hline
% SSLBackdoor & ImageNet & ImageNet-10 & - & - & 2.27 & 87.47 \\ \hline
% CorruptEncoder & ImageNet & ImageNet-10 & - & - & 1.61 & 84.94 \\ \bottomrule
% \end{tabular}
% }
% }
% \end{table}


































\begin{table*}[t]
\centering
    \caption{
    Performance of seed-sifting module TIS and the entire framework of T-Core against \textbf{adaptive attack}. 
     % The NPD of this experiment is 1250, the NFD is 62, and the Poi Num shows the results of TIS. 
    In this experiment, we construct universal adversarial perturbations (UAPs) that minimize the latent representation between the perturbed input and the samples from the target class across model layers. 
    Such UAPs are used as backdoor triggers for dataset poisoning.
    We test out the perturbation budget as 8, 16, 24, 32  of the infinite norm, respectively.
    `Poi Num' denotes the the number of poison are deems as clean seed data by TIS. 
   \review{ABCD}{Q1}}
    \resizebox{0.98\textwidth}{!}{\large
        \begin{tabular}{c|ccc|ccc|ccc|ccc}
    \toprule
    \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Perturbation\\ Range\end{tabular}} & \multicolumn{3}{c|}{8} & \multicolumn{3}{c|}{16} & \multicolumn{3}{c|}{24} & \multicolumn{3}{c}{32} \\ \cline{2-13} 
     & ACC & ASR & Poi Num & ACC & ASR & Poi Num & ACC & ASR & Poi Num & ACC & ASR & Poi Num \\ \midrule
    No Defense & 84.43 & 91.61 & - & 84.07 & 95.91 & - & 84.63 & 97.61 & - & 84.82 & 97.86 & - \\ \hline
    Ours & 81.61 & 2.36 & 0 & 82.13 & 2.99 & 0 & 82.92 & 4.71 & 2 & 82.04 & 5.52 & 1 \\ \bottomrule
    \end{tabular}
    }
\end{table*}





\begin{table*}[ht]
\caption{Performance of T-Core on Vision Transformer \textbf{ViT} against different types of backdoor threats of \threatone~(Dataset Poisoning), \threattwo~(Encoder Poisoning), and \threatthree~(Adaptive Poisoning). \review{ABD}{Q2}
}
\centering
\renewcommand{\arraystretch}{1.2}
\setlength{\tabcolsep}{4pt} % Adjust column spacing
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}lcccccc cccccc cccccc@{}}
\toprule
\multirow{2}{*}{Threat Type} & 
\multicolumn{6}{c}{\textbf{\threattwo} } & 
\multicolumn{4}{c}{\textbf{\threatone}  } & 
\multicolumn{4}{c}{\textbf{\threatthree} } \\ 
\cmidrule(lr){2-7} \cmidrule(lr){8-11} \cmidrule(l){12-15} 
& \multicolumn{2}{c}{BadNets} & 
\multicolumn{2}{c}{Blended} & 
\multicolumn{2}{c}{SIG} & 
\multicolumn{2}{c}{BadEncoder} & 
\multicolumn{2}{c}{DRUPE} & 
\multicolumn{2}{c}{BadEncoder} & 
\multicolumn{2}{c}{DRUPE} \\ 
\cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} 
\cmidrule(lr){8-9} \cmidrule(lr){10-11} 
\cmidrule(l){12-13} \cmidrule(l){14-15} \cmidrule(l){16-17} 
\cmidrule(l){18-19} 
& ACC$\uparrow$ & ASR$\downarrow$ & 
ACC$\uparrow$ & ASR$\downarrow$ & 
ACC$\uparrow$ & ASR$\downarrow$ & 
ACC$\uparrow$ & ASR$\downarrow$ & 
ACC$\uparrow$ & ASR$\downarrow$ & 
ACC$\uparrow$ & ASR$\downarrow$ & 
ACC$\uparrow$ & ASR$\downarrow$ \\ 
\midrule
No Defense & 72.17 & 87.57 & 72.09 & 82.53 & 72.03 & 62.99 & 60.33 & 98.79 & 66.22 & 99.83 & 58.02 & 99.99 & 66.20 & 99.99 \\ 
Ours & 70.94 & 4.35 & 70.91 & 3.55 & 70.94 & 3.15 & 56.46 & 0.26 & 64.95 & 4.50 & 55.55 & 2.50 & 65.25 & 5.57 \\ 
\bottomrule
\end{tabular}%
}
\label{tab:vit_performance}
\end{table*}


\begin{table*}[ht]
    \centering
    \caption{Performance of our seed-sifting module TIS on  Vision Transformer (\textbf{ViT}) against dataset poisoning of \threattwo, compared to other seed-sifting methods.
IBD-PSC is excluded because it relies on batch normalization, which ViT does not use. 
META-SIFT is omitted since we have not implemented it for ViT in time due to its complexity.
Poison rate is 20\% of the target class. \review{ABD}{Q2}
}
    \resizebox{0.8\textwidth}{!}{\large
    \begin{tabular}{c|c|c|c|c|c|c|c}
    \toprule
    \rowcolor[HTML]{FFFFFF} 
    \begin{tabular}[c]{@{}c@{}}Dataset\\ Poisoning\end{tabular} & BadNets & Blended & SIG & WaNet & TaCT & Adap-Blend & Adap-Patch \\ \midrule
    \rowcolor[HTML]{EFEFEF} 
    NPD & 125 & 125 & 100 & 125 & 125 & 125 & 125 \\ \hline
    \rowcolor[HTML]{EFEFEF} 
    NFD & 6 & 6 & 5 & 6 & 6 & 6 & 6 \\ \hline
    SCALE-UP & \cellcolor[HTML]{D9EAD3}0 & 3 & 3 & 2 & \cellcolor[HTML]{D9EAD3}0 & 1 & \cellcolor[HTML]{D9EAD3}0 \\ \hline
    Spectral & \cellcolor[HTML]{D9EAD3}0 & \cellcolor[HTML]{D9EAD3}0 & \cellcolor[HTML]{D9EAD3}0 & \cellcolor[HTML]{D9EAD3}0 & \cellcolor[HTML]{D9EAD3}0 & \cellcolor[HTML]{D9EAD3}0 & 1 \\ \hline
    SPECTRE & \cellcolor[HTML]{D9EAD3}0 & \cellcolor[HTML]{D9EAD3}0 & \cellcolor[HTML]{D9EAD3}0 & \cellcolor[HTML]{D9EAD3}0 & 1 & 1 & \cellcolor[HTML]{D9EAD3}0 \\ \hline
    Ours & \cellcolor[HTML]{D9EAD3}0 & \cellcolor[HTML]{D9EAD3}0 & \cellcolor[HTML]{D9EAD3}0 & \cellcolor[HTML]{D9EAD3}0 & \cellcolor[HTML]{D9EAD3}0 & \cellcolor[HTML]{D9EAD3}0 & \cellcolor[HTML]{D9EAD3}0 \\
\bottomrule
    \end{tabular}
    }
    \end{table*}



\begin{figure*}[ht]
\begin{center}
\begin{tcolorbox}[colback=lightgray!20, colframe=black, boxrule=0.5pt, arc=0pt, outer arc=0pt, boxsep=0pt, left=2pt, right=2pt, top=2pt, bottom=2pt]
\begin{minted}[
    linenos,                  % Show line numbers
    frame=lines,              % Add a border
    framesep=2mm,             % Space between border and code
    baselinestretch=1.2,      % Line spacing
    fontsize=\footnotesize    % Font size
]{python}
class MaskedLinear(nn.Module):
    def __init__(self, original_weight, mask, bias=None):
        super().__init__()
        self.original_weight = original_weight
        self.mask = mask  # Trainable mask initialized as all ones
        self.bias = bias

    def forward(self, x):
        # Clamp mask between 0 and 1
        self.mask.data.clamp_(0,1)
        masked_weight = self.original_weight * self.mask.unsqueeze(1)
        return torch.nn.functional.linear(x, masked_weight, self.bias)
\end{minted}
\end{tcolorbox}
\caption{Implementation of the \texttt{MaskedLinear} class, which applies a trainable mask to the weights of a linear layer. We use this code to transform a linear layer of \textbf{ViT} into a masked layer. The mask is clamped between 0 and 1 to ensure valid weight adjustments.
\review{ABD}{Q2}
}
\label{fig:masked_linear}
\end{center}
\end{figure*}













% \begin{table}[]
%     \caption{\textbf{Time expenses} (seconds) \textbf{in comparison} of different seed-sifting methods, on the CIFAR-10 dataset at varying dataset sizes per class. 
%   According to \cref{tab:clean_data_sifting,tab:clean_data_sifting_limited}, the faster IBD-PSC, SCALE-UP, and Spectral, generally perform poorly. 
%   Among the others, ours is the most efficient one. \review{ABCD}{Q4}
%     }
%     \resizebox{0.47\textwidth}{!}{\large
%     \begin{tabular}{c|c|c|c|c|c}
%     \toprule
%     \rowcolor[HTML]{BFBFBF} 
%     \textbf{\begin{tabular}[c]{@{}c@{}}Data Size\\ per Class\end{tabular}} & \textbf{100} & \textbf{500} & \textbf{1000} & \textbf{2500} & \textbf{5000} \\ \midrule
%     \textbf{IBD-PSC} & 3.83 & 14.94 & 26.81 & 64.81 & 139.69 \\ \hline
%     \textbf{SCALE-UP} & 0.69 & 3.02 & 6.00 & 14.81 & 29.51 \\ \hline
%     \textbf{Spectral} & \textbf{0.32} & \textbf{1.85} & \textbf{3.07} & \textbf{7.01} & \textbf{14.13} \\ \hline
%     \textbf{SPECTRE} & 14.53 & 74.23 & 117.95 & 231.71 & 456.57 \\ \hline
%     \textbf{META-SIFT} & 47.99 & 83.68 & 128.34 & 267.09 & 489.26 \\ \hline
%     \textbf{Ours} & 7.01 & 26.05 & 46.68 & 129.29 & 294.38 \\ \bottomrule
%     \end{tabular}
%     }
% \end{table}

% \begin{table}[t]
%     \caption{\textbf{Time expenses and memory usage} of Topological Invariance Sifting (TIS), Seed Expansion (SE), Encoder Channel Filtering (ECF), and Bootstrapping Learning (BL), in our T-Core method on CIFAR-10 dataset with ResNet18.\review{ABCD}{Q4}
%     }
%     \begin{tabular}{c|c|c|cl|c|c}
%     \toprule
%     Stages & TIS & SE & \multicolumn{2}{c|}{ECF} & BL & Total Expenses \\ \midrule
%     Time (s) & 294.4 & 60.1 & \multicolumn{2}{c|}{105.6} & 642.2 & 1102.3 \\ \midrule
%     VRAM (MB) & 5312 & 3338 & \multicolumn{2}{c|}{3484} & 4794 & 5312 \\ \bottomrule
%     \end{tabular}
% \end{table}




% \begin{table}[]
%     \caption{The \textbf{ablation on the hyper-parameters $\gamma_1$, $\gamma_2$} of bootstrapping learning. 
%     $\gamma_1$ is the selection rate from \textit{each class},  $\gamma_2$ is the selection rate from \textit{entire dataset}.
%     The results indicate that, compared to selection from the entire dataset, selection from \textit{each class} should be more cautious.
%     Also, the more cautious we are, the smaller the ASR. \review{ABCD}{Q3}
%     }
%     \resizebox{0.47\textwidth}{!}{\large
%     \begin{tabular}{ccccccccc}
%     \toprule
%     \multicolumn{9}{c}{\cellcolor[HTML]{CCCCCC}SIG} \\ \hline
%     \multicolumn{1}{c|}{\cellcolor[HTML]{CCCCCC}} & \multicolumn{4}{c|}{\cellcolor[HTML]{CCCCCC}\textbf{ACC$\uparrow$}} & \multicolumn{4}{c}{\cellcolor[HTML]{CCCCCC}\textbf{ASR$\downarrow$}} \\ \cline{2-9} 
%     \multicolumn{1}{c|}{\multirow{-2}{*}{\cellcolor[HTML]{CCCCCC}\textbf{No Defense}}} & \multicolumn{4}{c|}{\cellcolor[HTML]{CCCCCC}\textbf{84.72}} & \multicolumn{4}{c}{\cellcolor[HTML]{CCCCCC}\textbf{89.1}} \\ \midrule
%     \multicolumn{1}{c|}{\textbf{$\gamma_2$(\%)}} & \multicolumn{2}{c|}{\textbf{2}} & \multicolumn{2}{c|}{\textbf{5}} & \multicolumn{2}{c|}{\textbf{7}} & \multicolumn{2}{c}{\textbf{10}} \\ \hline
%     \multicolumn{1}{c|}{\textbf{$\gamma_1$(\%)}} & \multicolumn{1}{c|}{ACC$\uparrow$} & \multicolumn{1}{c|}{ASR$\downarrow$} & \multicolumn{1}{c|}{ACC$\uparrow$} & \multicolumn{1}{c|}{ASR$\downarrow$} & \multicolumn{1}{c|}{ACC$\uparrow$} & \multicolumn{1}{c|}{ASR$\downarrow$} & \multicolumn{1}{c|}{ACC$\uparrow$} & ASR$\downarrow$ \\ \hline
%     \multicolumn{1}{c|}{\textbf{1}} & \multicolumn{1}{c|}{88.24} & \multicolumn{1}{c|}{2.24} & \multicolumn{1}{c|}{88.36} & \multicolumn{1}{c|}{2.34} & \multicolumn{1}{c|}{87.79} & \multicolumn{1}{c|}{4.53} & \multicolumn{1}{c|}{87.22} & 7.92 \\ \hline
%     \multicolumn{1}{c|}{\textbf{2}} & \multicolumn{1}{c|}{89.09} & \multicolumn{1}{c|}{2.76} & \multicolumn{1}{c|}{87.31} & \multicolumn{1}{c|}{2.54} & \multicolumn{1}{c|}{86.91} & \multicolumn{1}{c|}{4.27} & \multicolumn{1}{c|}{87.13} & 8.44 \\ \hline
%     \multicolumn{1}{c|}{\textbf{5}} & \multicolumn{1}{c|}{87.98} & \multicolumn{1}{c|}{4.49} & \multicolumn{1}{c|}{86.16} & \multicolumn{1}{c|}{9.59} & \multicolumn{1}{c|}{83.55} & \multicolumn{1}{c|}{21.73} & \multicolumn{1}{c|}{81.84} & 40.57 \\ \midrule
%     \multicolumn{9}{c}{\cellcolor[HTML]{CCCCCC}Blended} \\ \hline
%     \multicolumn{1}{c|}{\cellcolor[HTML]{CCCCCC}} & \multicolumn{4}{c|}{\cellcolor[HTML]{CCCCCC}\textbf{ACC$\uparrow$}} & \multicolumn{4}{c}{\cellcolor[HTML]{CCCCCC}\textbf{ASR$\downarrow$}} \\ \cline{2-9} 
%     \multicolumn{1}{c|}{\multirow{-2}{*}{\cellcolor[HTML]{CCCCCC}\textbf{No Defense}}} & \multicolumn{4}{c|}{\cellcolor[HTML]{CCCCCC}\textbf{84.84}} & \multicolumn{4}{c}{\cellcolor[HTML]{CCCCCC}\textbf{89.12}} \\ \midrule
%     \multicolumn{1}{c|}{\textbf{$\gamma_2$(\%)}} & \multicolumn{2}{c|}{\textbf{2}} & \multicolumn{2}{c|}{\textbf{5}} & \multicolumn{2}{c|}{\textbf{7}} & \multicolumn{2}{c}{\textbf{10}} \\ \hline
%     \multicolumn{1}{c|}{\textbf{$\gamma_1$(\%)}} & \multicolumn{1}{c|}{ACC$\uparrow$} & \multicolumn{1}{c|}{ASR$\downarrow$} & \multicolumn{1}{c|}{ACC$\uparrow$} & \multicolumn{1}{c|}{ASR$\downarrow$} & \multicolumn{1}{c|}{ACC$\uparrow$} & \multicolumn{1}{c|}{ASR$\downarrow$} & \multicolumn{1}{c|}{ACC$\uparrow$} & ASR$\downarrow$ \\ \hline
%     \multicolumn{1}{c|}{\textbf{1}} & \multicolumn{1}{c|}{88.64} & \multicolumn{1}{c|}{4.48} & \multicolumn{1}{c|}{87.38} & \multicolumn{1}{c|}{4.93} & \multicolumn{1}{c|}{88.01} & \multicolumn{1}{c|}{6.37} & \multicolumn{1}{c|}{86.93} & 13.75 \\ \hline
%     \multicolumn{1}{c|}{\textbf{2}} & \multicolumn{1}{c|}{88.09} & \multicolumn{1}{c|}{4.43} & \multicolumn{1}{c|}{87.35} & \multicolumn{1}{c|}{5.9} & \multicolumn{1}{c|}{87.14} & \multicolumn{1}{c|}{7.37} & \multicolumn{1}{c|}{86.26} & 16.07 \\ \hline
%     \multicolumn{1}{c|}{\textbf{5}} & \multicolumn{1}{c|}{86.63} & \multicolumn{1}{c|}{8.46} & \multicolumn{1}{c|}{85.31} & \multicolumn{1}{c|}{12.74} & \multicolumn{1}{c|}{83.21} & \multicolumn{1}{c|}{26.07} & \multicolumn{1}{c|}{82.55} & 44.15 \\ \bottomrule
%     \end{tabular}
%     }
%     \end{table}

% \begin{table}[]
% \caption{The \textbf{ablation on the bootstrapping rate} $\rho$ in \cref{algo:bootstrapping_learning}, \textit{i.e.}, when we choose to halt the bootstrapping learning.
% `Poi Num' denotes the final number of poison samples that are included for training. 
% We use dataset poisoning of SIG and Blended on CIFAR-10,  the poison rate is the default 20\% of the target class. \review{ABCD}{Q3}
% }
%  \resizebox{0.47\textwidth}{!}{\large
%     \begin{tabular}{c|ccc|ccc}
%     \toprule
%     \rowcolor[HTML]{CCCCCC} 
%     \cellcolor[HTML]{CCCCCC} & \multicolumn{3}{c|}{\cellcolor[HTML]{CCCCCC}SIG} & \multicolumn{3}{c}{\cellcolor[HTML]{CCCCCC}Blended} \\ \cline{2-7} 
%     \rowcolor[HTML]{CCCCCC} 
%     \multirow{-2}{*}{\cellcolor[HTML]{CCCCCC}\begin{tabular}[c]{@{}c@{}}Bootstrapping\\ Rate(\%)\end{tabular}} & \multicolumn{1}{c|}{\cellcolor[HTML]{CCCCCC}ACC$\uparrow$} & \multicolumn{1}{c|}{\cellcolor[HTML]{CCCCCC}ASR$\downarrow$} & Poi Num & \multicolumn{1}{c|}{\cellcolor[HTML]{CCCCCC}ACC$\uparrow$} & \multicolumn{1}{c|}{\cellcolor[HTML]{CCCCCC}ASR$\downarrow$} & Poi Num \\ \hline
%     \rowcolor[HTML]{CCCCCC} 
%     No Defense & \multicolumn{1}{c|}{\cellcolor[HTML]{CCCCCC}84.72} & \multicolumn{1}{c|}{\cellcolor[HTML]{CCCCCC}89.10} & - & \multicolumn{1}{c|}{\cellcolor[HTML]{CCCCCC}84.84} & \multicolumn{1}{c|}{\cellcolor[HTML]{CCCCCC}89.12} & - \\ \midrule
%     97 & \multicolumn{1}{c|}{85.13} & \multicolumn{1}{c|}{12.48} & 65 & \multicolumn{1}{c|}{85.54} & \multicolumn{1}{c|}{71.54} & 568 \\ \hline
%     95 & \multicolumn{1}{c|}{87.62} & \multicolumn{1}{c|}{3.11} & 9 & \multicolumn{1}{c|}{86.62} & \multicolumn{1}{c|}{79.38} & 88 \\ \hline
%     90 & \multicolumn{1}{c|}{87.31} & \multicolumn{1}{c|}{2.54} & 0 & \multicolumn{1}{c|}{87.35} & \multicolumn{1}{c|}{5.90} & 13 \\ \hline
%     85 & \multicolumn{1}{c|}{81.09} & \multicolumn{1}{c|}{1.87} & 0 & \multicolumn{1}{c|}{82.26} & \multicolumn{1}{c|}{3.71} & 5 \\ \hline
%     80 & \multicolumn{1}{c|}{79.41} & \multicolumn{1}{c|}{2.06} & 0 & \multicolumn{1}{c|}{80.63} & \multicolumn{1}{c|}{2.31} & 0 \\ \hline
%     70 & \multicolumn{1}{c|}{76.22} & \multicolumn{1}{c|}{1.63} & 0 & \multicolumn{1}{c|}{77.10} & \multicolumn{1}{c|}{1.56} & 0 \\ \bottomrule
%     \end{tabular}
%     }
%     \end{table}



\begin{table*}[htbp]
    \centering
    \begin{minipage}[t]{0.48\textwidth}
        \centering
        \caption{The \textbf{ablation on the hyper-parameters $\gamma_1$, $\gamma_2$} of bootstrapping learning. 
        $\gamma_1$ is the selection rate from \textit{each class},  $\gamma_2$ is the selection rate from \textit{entire dataset}.
        The results indicate that, compared to selection from the entire dataset, selection from \textit{each class} should be more cautious.
        Also, the more cautious we are, the smaller the ASR. \review{ABCD}{Q3}
        }
        \resizebox{\textwidth}{!}{\large
        \begin{tabular}{ccccccccc}
        \toprule
        \multicolumn{9}{c}{\cellcolor[HTML]{FFFFFF}SIG} \\ \hline
        \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}} & \multicolumn{4}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{ACC$\uparrow$}} & \multicolumn{4}{c}{\cellcolor[HTML]{FFFFFF}\textbf{ASR$\downarrow$}} \\ \cline{2-9} 
        \multicolumn{1}{c|}{\multirow{-2}{*}{\cellcolor[HTML]{FFFFFF}\textbf{No Defense}}} & \multicolumn{4}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{84.72}} & \multicolumn{4}{c}{\cellcolor[HTML]{FFFFFF}\textbf{89.1}} \\ \midrule
        \multicolumn{1}{c|}{\textbf{$\gamma_2$(\%)}} & \multicolumn{2}{c|}{\textbf{2}} & \multicolumn{2}{c|}{\textbf{5}} & \multicolumn{2}{c|}{\textbf{7}} & \multicolumn{2}{c}{\textbf{10}} \\ \hline
        \multicolumn{1}{c|}{\textbf{$\gamma_1$(\%)}} & \multicolumn{1}{c|}{ACC$\uparrow$} & \multicolumn{1}{c|}{ASR$\downarrow$} & \multicolumn{1}{c|}{ACC$\uparrow$} & \multicolumn{1}{c|}{ASR$\downarrow$} & \multicolumn{1}{c|}{ACC$\uparrow$} & \multicolumn{1}{c|}{ASR$\downarrow$} & \multicolumn{1}{c|}{ACC$\uparrow$} & ASR$\downarrow$ \\ \hline
        \multicolumn{1}{c|}{\textbf{1}} & \multicolumn{1}{c|}{88.24} & \multicolumn{1}{c|}{2.24} & \multicolumn{1}{c|}{88.36} & \multicolumn{1}{c|}{2.34} & \multicolumn{1}{c|}{87.79} & \multicolumn{1}{c|}{4.53} & \multicolumn{1}{c|}{87.22} & 7.92 \\ \hline
        \multicolumn{1}{c|}{\textbf{2}} & \multicolumn{1}{c|}{89.09} & \multicolumn{1}{c|}{2.76} & \multicolumn{1}{c|}{87.31} & \multicolumn{1}{c|}{2.54} & \multicolumn{1}{c|}{86.91} & \multicolumn{1}{c|}{4.27} & \multicolumn{1}{c|}{87.13} & 8.44 \\ \hline
        \multicolumn{1}{c|}{\textbf{5}} & \multicolumn{1}{c|}{87.98} & \multicolumn{1}{c|}{4.49} & \multicolumn{1}{c|}{86.16} & \multicolumn{1}{c|}{9.59} & \multicolumn{1}{c|}{83.55} & \multicolumn{1}{c|}{21.73} & \multicolumn{1}{c|}{81.84} & 40.57 \\ \midrule
        \multicolumn{9}{c}{\cellcolor[HTML]{FFFFFF}Blended} \\ \hline
        \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}} & \multicolumn{4}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{ACC$\uparrow$}} & \multicolumn{4}{c}{\cellcolor[HTML]{FFFFFF}\textbf{ASR$\downarrow$}} \\ \cline{2-9} 
        \multicolumn{1}{c|}{\multirow{-2}{*}{\cellcolor[HTML]{FFFFFF}\textbf{No Defense}}} & \multicolumn{4}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{84.84}} & \multicolumn{4}{c}{\cellcolor[HTML]{FFFFFF}\textbf{89.12}} \\ \midrule
        \multicolumn{1}{c|}{\textbf{$\gamma_2$(\%)}} & \multicolumn{2}{c|}{\textbf{2}} & \multicolumn{2}{c|}{\textbf{5}} & \multicolumn{2}{c|}{\textbf{7}} & \multicolumn{2}{c}{\textbf{10}} \\ \hline
        \multicolumn{1}{c|}{\textbf{$\gamma_1$(\%)}} & \multicolumn{1}{c|}{ACC$\uparrow$} & \multicolumn{1}{c|}{ASR$\downarrow$} & \multicolumn{1}{c|}{ACC$\uparrow$} & \multicolumn{1}{c|}{ASR$\downarrow$} & \multicolumn{1}{c|}{ACC$\uparrow$} & \multicolumn{1}{c|}{ASR$\downarrow$} & \multicolumn{1}{c|}{ACC$\uparrow$} & ASR$\downarrow$ \\ \hline
        \multicolumn{1}{c|}{\textbf{1}} & \multicolumn{1}{c|}{88.64} & \multicolumn{1}{c|}{4.48} & \multicolumn{1}{c|}{87.38} & \multicolumn{1}{c|}{4.93} & \multicolumn{1}{c|}{88.01} & \multicolumn{1}{c|}{6.37} & \multicolumn{1}{c|}{86.93} & 13.75 \\ \hline
        \multicolumn{1}{c|}{\textbf{2}} & \multicolumn{1}{c|}{88.09} & \multicolumn{1}{c|}{4.43} & \multicolumn{1}{c|}{87.35} & \multicolumn{1}{c|}{5.9} & \multicolumn{1}{c|}{87.14} & \multicolumn{1}{c|}{7.37} & \multicolumn{1}{c|}{86.26} & 16.07 \\ \hline
        \multicolumn{1}{c|}{\textbf{5}} & \multicolumn{1}{c|}{86.63} & \multicolumn{1}{c|}{8.46} & \multicolumn{1}{c|}{85.31} & \multicolumn{1}{c|}{12.74} & \multicolumn{1}{c|}{83.21} & \multicolumn{1}{c|}{26.07} & \multicolumn{1}{c|}{82.55} & 44.15 \\ \bottomrule
        \end{tabular}
        }
    \end{minipage}
    \hfill
    \begin{minipage}[t]{0.48\textwidth}
        \centering
        \caption{The \textbf{ablation on the bootstrapping rate} $\rho$ in \cref{algo:bootstrapping_learning} Bootstrapping Learning, \textit{i.e.}, when we choose to halt the bootstrapping learning.
        `Poi Num' denotes the final number of poison samples that are included for training. 
        We use dataset poisoning of SIG and Blended on CIFAR-10,  the poison rate is the default 20\% of the target class. \review{ABCD}{Q3}
        }
        \vspace{5mm}
        \resizebox{\textwidth}{!}{\large
        \begin{tabular}{c|ccc|ccc}
        \toprule
        \rowcolor[HTML]{FFFFFF} 
        \cellcolor[HTML]{FFFFFF} & \multicolumn{3}{c|}{\cellcolor[HTML]{FFFFFF}SIG} & \multicolumn{3}{c}{\cellcolor[HTML]{FFFFFF}Blended} \\ \cline{2-7} 
        \rowcolor[HTML]{FFFFFF} 
        \multirow{-2}{*}{\cellcolor[HTML]{FFFFFF}\begin{tabular}[c]{@{}c@{}}Bootstrapping\\ Rate(\%)\end{tabular}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}ACC$\uparrow$} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}ASR$\downarrow$} & Poi Num & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}ACC$\uparrow$} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}ASR$\downarrow$} & Poi Num \\ \hline
        \rowcolor[HTML]{FFFFFF} 
        No Defense & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}84.72} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}89.10} & - & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}84.84} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}89.12} & - \\ \midrule
        97 & \multicolumn{1}{c|}{85.13} & \multicolumn{1}{c|}{12.48} & 65 & \multicolumn{1}{c|}{85.54} & \multicolumn{1}{c|}{71.54} & 568 \\ \hline
        95 & \multicolumn{1}{c|}{87.62} & \multicolumn{1}{c|}{3.11} & 9 & \multicolumn{1}{c|}{86.62} & \multicolumn{1}{c|}{79.38} & 88 \\ \hline
        90 & \multicolumn{1}{c|}{87.31} & \multicolumn{1}{c|}{2.54} & 0 & \multicolumn{1}{c|}{87.35} & \multicolumn{1}{c|}{5.90} & 13 \\ \hline
        85 & \multicolumn{1}{c|}{81.09} & \multicolumn{1}{c|}{1.87} & 0 & \multicolumn{1}{c|}{82.26} & \multicolumn{1}{c|}{3.71} & 5 \\ \hline
        80 & \multicolumn{1}{c|}{79.41} & \multicolumn{1}{c|}{2.06} & 0 & \multicolumn{1}{c|}{80.63} & \multicolumn{1}{c|}{2.31} & 0 \\ \hline
        70 & \multicolumn{1}{c|}{76.22} & \multicolumn{1}{c|}{1.63} & 0 & \multicolumn{1}{c|}{77.10} & \multicolumn{1}{c|}{1.56} & 0 \\ \bottomrule
        \end{tabular}
        }
    \end{minipage}
\end{table*}






















































\begin{table*}[htbp]
    \centering
    \begin{minipage}[t]{0.45\textwidth}
            \caption{\textbf{Time expenses} (seconds) \textbf{in comparison} of different seed-sifting methods, on the CIFAR-10 dataset at varying dataset sizes per class. 
  According to \cref{tab:clean_data_sifting,tab:clean_data_sifting_limited}, the faster IBD-PSC, SCALE-UP, and Spectral, generally perform poorly. 
  Among the others, ours is the most efficient one. \review{ABCD}{Q4}
    }
        \centering
        \resizebox{\textwidth}{!}{\large
        \begin{tabular}{c|c|c|c|c|c}
        \toprule
        %\rowcolor[HTML]{BFBFBF} 
        \rowcolor[HTML]{FFFFFF}
        \textbf{\begin{tabular}[c]{@{}c@{}}Data Size\\ per Class\end{tabular}} & \textbf{100} & \textbf{500} & \textbf{1000} & \textbf{2500} & \textbf{5000} \\ \midrule
        \textbf{IBD-PSC} & 3.83 & 14.94 & 26.81 & 64.81 & 139.69 \\ \hline
        \textbf{SCALE-UP} & 0.69 & 3.02 & 6.00 & 14.81 & 29.51 \\ \hline
        \textbf{Spectral} & \textbf{0.32} & \textbf{1.85} & \textbf{3.07} & \textbf{7.01} & \textbf{14.13} \\ \hline
        \textbf{SPECTRE} & 14.53 & 74.23 & 117.95 & 231.71 & 456.57 \\ \hline
        \textbf{META-SIFT} & 47.99 & 83.68 & 128.34 & 267.09 & 489.26 \\ \hline
        \textbf{Ours} & 7.01 & 26.05 & 46.68 & 129.29 & 294.38 \\ \bottomrule
        \end{tabular}
        }
    \end{minipage}
    \hfill
    \begin{minipage}[t]{0.45\textwidth}
        \caption{\textbf{Time expenses and memory usage} of Topological Invariance Sifting (TIS), Seed Expansion (SE), Encoder Channel Filtering (ECF), and Bootstrapping Learning (BL), in our T-Core method on CIFAR-10 dataset with ResNet18.\review{ABCD}{Q4}
    }
        \vspace{5mm}
        \centering
        \begin{tabular}{c|c|c|cl|c|c}
        \toprule
        Stages & TIS & SE & \multicolumn{2}{c|}{ECF} & BL & Total Expenses \\ \midrule
        Time (s) & 294.4 & 60.1 & \multicolumn{2}{c|}{105.6} & 642.2 & 1102.3 \\ \midrule
        VRAM (MB) & 5312 & 3338 & \multicolumn{2}{c|}{3484} & 4794 & 5312 \\ \bottomrule
        \end{tabular}
    \end{minipage}
\end{table*}




% \begin{table}[]
%     \centering
%     \caption{The \textbf{ablation on the unlearning} process of \cref{eq:selective_unlearning}. 
%     We conduct Encoder Channel Filtering against encoder poisoning of BadEncoder.
%     Here we use different hard mask thresholds to better illustrate the difference w/wo Unlearning process.
%     We report the number of Channels deemed as untrusted through different mask thresholding, as well as the ASR and ACC of the corresponding models pruned with the untrusted channels. {\color{red} \underline {[Review \#A, Q6]}}
%     }
%     \resizebox{0.47\textwidth}{!}{\large
%     \begin{tabular}{c|c|c|cc}
%     \toprule
%      &  & \begin{tabular}[c]{@{}c@{}}Number of Channels\\ deemed as Untrusted\end{tabular} & ACC$\uparrow$ & ASR$\downarrow$ \\ \cline{3-5} 
%     \multirow{-2}{*}{w/wo Unlearning} & \multirow{-2}{*}{Mask Threshold} & No Defense (0) & 82.83 & 99.37 \\ \hline
%     \cref{eq:selective_unlearning} + \cref{eq:filter_recovery}  & 0 & 116 & 80.18 & 1.13 \\ \hline
%      & \cellcolor[HTML]{F2F2F2} $<$ 0.7 & \cellcolor[HTML]{F2F2F2}0 & \cellcolor[HTML]{F2F2F2}82.83 & \cellcolor[HTML]{F2F2F2}99.37 \\ \cline{2-5} 
%      & 0.7 & 71 & 52.75 & 96.54 \\ \cline{2-5} 
%      & 0.8 & 223 & 30.75 & 78.16 \\ \cline{2-5} 
%     \multirow{-4}{*}{\begin{tabular}[c]{@{}c@{}}
%     \cref{eq:filter_recovery} only
%     \end{tabular}} & 0.9 & 651 & 15.05 & 0.14 \\ \bottomrule
%     \end{tabular}
%     }
% \end{table}

% \begin{table}[]
% \caption{The \textbf{ablation on the expansion ratio} used in \cref{algo:seedexpansion}, where each expansion ratio is used to continue the following process of T-Core and obtain the final model. We report the ASR and ACC of each resulting model for comparison. We conduct this experiment on dataset poisoning of SIG and Blended on CIFAR-10 under \threattwo. \review{A}{Q7}
% }.
%  \resizebox{0.47\textwidth}{!}{\large
%     \begin{tabular}{c|cc|cc}
%     \toprule
%     \rowcolor[HTML]{CCCCCC} 
%     \cellcolor[HTML]{CCCCCC} & \multicolumn{2}{c|}{\cellcolor[HTML]{CCCCCC}SIG} & \multicolumn{2}{c}{\cellcolor[HTML]{CCCCCC}Blended} \\ \cline{2-5} 
%     \rowcolor[HTML]{CCCCCC} 
%     \multirow{-2}{*}{\cellcolor[HTML]{CCCCCC}\begin{tabular}[c]{@{}c@{}}Expansion\\ Rate\end{tabular}} & \multicolumn{1}{c|}{\cellcolor[HTML]{CCCCCC}ACC$\uparrow$} & ASR$\downarrow$ & \multicolumn{1}{c|}{\cellcolor[HTML]{CCCCCC}ACC$\uparrow$} & ASR$\downarrow$ \\ \hline
%     \rowcolor[HTML]{CCCCCC} 
%     No Defense & \multicolumn{1}{c|}{\cellcolor[HTML]{CCCCCC}84.72} & 89.10 & \multicolumn{1}{c|}{\cellcolor[HTML]{CCCCCC}84.84} & 89.12 \\ \midrule
%     10\% & \multicolumn{1}{c|}{87.48} & 0.31 & \multicolumn{1}{c|}{83.11} & 11.03 \\ \hline
%     20\% & \multicolumn{1}{c|}{87.31} & 2.54 & \multicolumn{1}{c|}{87.35} & 5.90 \\ \hline
%     30\% & \multicolumn{1}{c|}{86.92} & 4.21 & \multicolumn{1}{c|}{85.39} & 13.48 \\ \hline
%     40\% & \multicolumn{1}{c|}{87.59} & 6.10 & \multicolumn{1}{c|}{82.98} & 32.87 \\ \bottomrule
%     \end{tabular}
%     }
% \end{table}

\begin{table*}[htbp]
    \centering
    % 第一个minipage
    \begin{minipage}[t]{0.48\textwidth}
        \centering
        \caption{The \textbf{ablation on the unlearning} process of \cref{eq:selective_unlearning}. 
        We conduct Encoder Channel Filtering against encoder poisoning of BadEncoder.
        Here we use different hard mask thresholds to better illustrate the difference w/wo Unlearning process.
        We report the number of Channels deemed as untrusted through different mask thresholding, as well as the ASR and ACC of the corresponding models pruned with the untrusted channels. {\color{red} \underline {[Review \#A, Q6]}}
        }
        \vspace{26pt}
        \resizebox{\textwidth}{!}{\large
        \begin{tabular}{c|c|c|cc}
        \toprule
         &  & \begin{tabular}[c]{@{}c@{}}Number of Channels\\ deemed as Untrusted\end{tabular} & ACC$\uparrow$ & ASR$\downarrow$ \\ \cline{3-5} 
        \multirow{-2}{*}{w/wo Unlearning} & \multirow{-2}{*}{Mask Threshold} & No Defense (0) & 82.83 & 99.37 \\ \hline
        \cref{eq:selective_unlearning} + \cref{eq:filter_recovery}  & 0 & 116 & 80.18 & 1.13 \\ \hline
         & \cellcolor[HTML]{F2F2F2} $<$ 0.7 & \cellcolor[HTML]{F2F2F2}0 & \cellcolor[HTML]{F2F2F2}82.83 & \cellcolor[HTML]{F2F2F2}99.37 \\ \cline{2-5} 
         & 0.7 & 71 & 52.75 & 96.54 \\ \cline{2-5} 
         & 0.8 & 223 & 30.75 & 78.16 \\ \cline{2-5} 
        \multirow{-4}{*}{\begin{tabular}[c]{@{}c@{}}\cref{eq:filter_recovery} only\end{tabular}} & 0.9 & 651 & 15.05 & 0.14 \\ \bottomrule
        \end{tabular}
        }
    \end{minipage}
    \hfill 
    \begin{minipage}[t]{0.48\textwidth}
        \centering
        \caption{The \textbf{ablation on the expansion ratio} used in \cref{algo:seedexpansion}, where each expansion ratio is used to continue the following process of T-Core and obtain the final model. We report the ASR and ACC of each resulting model for comparison. We conduct this experiment on dataset poisoning of SIG and Blended on CIFAR-10 under \threattwo. \review{A}{Q7}
        }
        \resizebox{\textwidth}{!}{\large
        \begin{tabular}{c|cc|cc}
        \toprule
        \rowcolor[HTML]{FFFFFF} 
        \cellcolor[HTML]{FFFFFF} & \multicolumn{2}{c|}{\cellcolor[HTML]{FFFFFF}SIG} & \multicolumn{2}{c}{\cellcolor[HTML]{FFFFFF}Blended} \\ \cline{2-5} 
        \rowcolor[HTML]{FFFFFF} 
        \multirow{-2}{*}{\cellcolor[HTML]{FFFFFF}\begin{tabular}[c]{@{}c@{}}Expansion\\ Rate\end{tabular}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}ACC$\uparrow$} & ASR$\downarrow$ & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}ACC$\uparrow$} & ASR$\downarrow$ \\ \hline
        \rowcolor[HTML]{FFFFFF} 
        No Defense & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}84.72} & 89.10 & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}84.84} & 89.12 \\ \midrule
        10\% & \multicolumn{1}{c|}{87.48} & 0.31 & \multicolumn{1}{c|}{83.11} & 11.03 \\ \hline
        20\% & \multicolumn{1}{c|}{87.31} & 2.54 & \multicolumn{1}{c|}{87.35} & 5.90 \\ \hline
        30\% & \multicolumn{1}{c|}{86.92} & 4.21 & \multicolumn{1}{c|}{85.39} & 13.48 \\ \hline
        40\% & \multicolumn{1}{c|}{87.59} & 6.10 & \multicolumn{1}{c|}{82.98} & 32.87 \\ \bottomrule
        \end{tabular}
        }
    \end{minipage}
\end{table*}







\begin{figure*}[htbp]
    \centering
    \includegraphics[width=1.0\textwidth]{images/CT_ablation.pdf} 
    \caption{Number of poison samples in the largest loss region of the target class after seed expansion.
    Experiments are conducted on 7 dataset poisoning attacks at poison ratios of 0.1, 0.2, 0.3, and 0.4 for the target class. \review{A}{Q5}}
\end{figure*}











\begin{table*}[htbp]
    \centering
    \caption{Performance of our T-Core Method in the presence of \textbf{multiple dataset poisoning} on CIFAR-10 Dataset.
    In each setting of this experiment, Blended, TaCT, and BadNets use 1250 poison samples each, while SIG has 1000.
    For TIS, we use the default seed selection ratio of 1\%.
    `Poison in Seed' means how many poison samples are sifted out as seed data. \review{A}{Q8}
    }
    \label{tab:poisoning_performance}
    \resizebox{\textwidth}{!}{%
    \begin{tabular}{lcccccccc}
        \toprule
        \multirow{2}{*}{Dataset Poisoning} & \multicolumn{3}{c}{No Defense} & \multicolumn{4}{c}{Our Defense (T-Core)} \\
        \cmidrule(lr){2-4} \cmidrule(lr){5-8}
         & ASR1 (\%) & ASR2 (\%) & ACC (\%) & ASR1 (\%) & ASR2 (\%) & ACC (\%) & Poison in Seed \\
        \midrule
        Blended \& SIG & 85.99 & 86.41 & 84.26 & 6.16 & 5.24 & 81.94 & 0 \\
        TaCT \& SIG    & 91.40 & 89.49 & 84.06 & 1.70 & 3.44 & 80.65 & 0 \\
        BadNets \& SIG & 96.26 & 90.27 & 84.32 & 2.89 & 4.20 & 81.76 & 0 \\
        \bottomrule
    \end{tabular}
    }
\end{table*}




\begin{table*}[]
    \centering 
    \caption{Number of poisoned samples in the sifted-out samples (deemed clean) from poisoned datasets with varying selected seed ratios (0.1, 0.15, 0.2, 0.25, 0.3) in the target class for different seed-sifting methods. 
    We use different limited sizes of CIFAR-10 datasets (100 to 400 per class), representing \textbf{more realistic TL settings}. ND denotes the \uline{\textit{ number of total data} per class}, 
    NPD denotes the \uline{\textit{number of poisoned data} in the target class} with a default poison ratio of 20\%, and NFD denotes the \uline{\textit{number of filtered data} in the target class deemed clean}. 
    We use SIG attack for this experiment, more will be provided in a revision. \review{B}{Q9}
    }
    \resizebox{\textwidth}{!}{%
    \begin{tabular}{c|ccccc|ccccc|ccccc|ccccc}
    \toprule
    \rowcolor[HTML]{FFFFFF} 
    \textbf{\begin{tabular}[c]{@{}c@{}} ND\end{tabular}} & \multicolumn{5}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{100}} & \multicolumn{5}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{200}} & \multicolumn{5}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{300}} & \multicolumn{5}{c}{\cellcolor[HTML]{FFFFFF}\textbf{400}} \\ \hline
    \rowcolor[HTML]{FFFFFF} 
    \textbf{Seed Rate} & \textbf{0.1} & \textbf{0.15} & \textbf{0.2} & \textbf{0.25} & \textbf{0.3} & \textbf{0.1} & \textbf{0.15} & \textbf{0.2} & \textbf{0.25} & \textbf{0.3} & \textbf{0.1} & \textbf{0.15} & \textbf{0.2} & \textbf{0.25} & \textbf{0.3} & \textbf{0.1} & \textbf{0.15} & \textbf{0.2} & \textbf{0.25} & \textbf{0.3} \\ \midrule
    \rowcolor[HTML]{EFEFEF} 
    \textbf{NPD} & \multicolumn{5}{c|}{\cellcolor[HTML]{EFEFEF}20} & \multicolumn{5}{c|}{\cellcolor[HTML]{EFEFEF}40} & \multicolumn{5}{c|}{\cellcolor[HTML]{EFEFEF}60} & \multicolumn{5}{c}{\cellcolor[HTML]{EFEFEF}80} \\ \midrule
    \rowcolor[HTML]{EFEFEF} 
    \textbf{NFD} & 10 & 15 & 20 & 25 & 30 & 20 & 30 & 40 & 50 & 60 & 30 & 45 & 60 & 75 & 90 & 40 & 60 & 80 & 100 & 120 \\ \midrule
    % \textbf{Seed Num} & 100 & 150 & 200 & 250 & 300 & 200 & 300 & 400 & 500 & 600 & 300 & 450 & 600 & 750 & 900 & 400 & 600 & 800 & 1000 & 1200 \\ \midrule
    \textbf{IBD-PSC} & 1 & 4 & 5 & 6 & 7 & 2 & 5 & 5 & 6 & 7 & 1 & 2 & 6 & 13 & 18 & 2 & 3 & 7 & 10 & 13 \\ \midrule
    \textbf{SCALE-UP} & 1 & 2 & 2 & 4 & 4 & 1 & 1 & 3 & 7 & 8 & 6 & 9 & 11 & 14 & 16 & 7 & 10 & 13 & 17 & 23 \\ \midrule
    \textbf{Spectral} & \cellcolor[HTML]{D9EAD3}0 & 1 & 1 & 2 & 2 & 1 & 1 & 2 & 2 & 3 & 2 & 2 & 3 & 3 & 3 & 4 & 5 & 5 & 7 & 7 \\ \midrule
    \textbf{SPECTRE} & \cellcolor[HTML]{D9EAD3}0 & \cellcolor[HTML]{D9EAD3}0 & \cellcolor[HTML]{D9EAD3}0 & \cellcolor[HTML]{D9EAD3}0 & \cellcolor[HTML]{D9EAD3}0 & \cellcolor[HTML]{D9EAD3}0 & \cellcolor[HTML]{D9EAD3}0 & \cellcolor[HTML]{D9EAD3}0 & \cellcolor[HTML]{D9EAD3}0 & \cellcolor[HTML]{D9EAD3}0 & 1 & 1 & 1 & 1 & 1 & \cellcolor[HTML]{D9EAD3}0 & \cellcolor[HTML]{D9EAD3}0 & 1 & 2 & 4 \\ \midrule
    \textbf{META-SIFT} & 2 & 3 & 6 & 7 & 7 & 5 & 5 & 6 & 7 & 8 & 11 & 13 & 18 & 19 & 19 & 6 & 7 & 13 & 15 & 17 \\ \midrule
    \textbf{Ours} & \cellcolor[HTML]{D9EAD3}0 & \cellcolor[HTML]{D9EAD3}0 & \cellcolor[HTML]{D9EAD3}0 & \cellcolor[HTML]{D9EAD3}0 & 1 & \cellcolor[HTML]{D9EAD3}0 & \cellcolor[HTML]{D9EAD3}0 & \cellcolor[HTML]{D9EAD3}0 & \cellcolor[HTML]{D9EAD3}0 & \cellcolor[HTML]{D9EAD3}0 & \cellcolor[HTML]{D9EAD3}0 & \cellcolor[HTML]{D9EAD3}0 & \cellcolor[HTML]{D9EAD3}0 & \cellcolor[HTML]{D9EAD3}0 & \cellcolor[HTML]{D9EAD3}0 & \cellcolor[HTML]{D9EAD3}0 & \cellcolor[HTML]{D9EAD3}0 & \cellcolor[HTML]{D9EAD3}0 & \cellcolor[HTML]{D9EAD3}0 & \cellcolor[HTML]{D9EAD3}0 \\ \bottomrule
    \end{tabular}
    }
    \label{tab:clean_data_sifting_limited}
\end{table*}
\clearpage



































% \begin{table}[]
%     \caption{Performance of our T-Core Method in the presence of \textbf{multiple dataset poisoning} on CIFAR-10 Dataset. 
%     NPD means the number of the poison samples 
%     }
%     \resizebox{0.47\textwidth}{!}{\large
%     \begin{tabular}{c|ccc|ccc|ccc}
%     \toprule
%     \rowcolor[HTML]{CCCCCC} 
%     \cellcolor[HTML]{CCCCCC}{\color[HTML]{08090C} } & \multicolumn{3}{c|}{\cellcolor[HTML]{CCCCCC}Blended \& SIG} & \multicolumn{3}{c|}{\cellcolor[HTML]{CCCCCC}TaCT \& SIG} & \multicolumn{3}{c}{\cellcolor[HTML]{CCCCCC}BadNets \& SIG} \\ \cline{2-10} 
%     \rowcolor[HTML]{CCCCCC} 
%     \multirow{-2}{*}{\cellcolor[HTML]{CCCCCC}{\color[HTML]{08090C} \begin{tabular}[c]{@{}c@{}}Dataset\\ Poisoning\end{tabular}}} & \multicolumn{1}{c|}{\cellcolor[HTML]{CCCCCC}Blended ASR} & \multicolumn{1}{c|}{\cellcolor[HTML]{CCCCCC}SIG ASR} & ACC & \multicolumn{1}{c|}{\cellcolor[HTML]{CCCCCC}TaCT ASR} & \multicolumn{1}{c|}{\cellcolor[HTML]{CCCCCC}SIG ASR} & ACC & \multicolumn{1}{c|}{\cellcolor[HTML]{CCCCCC}BadNets ASR} & \multicolumn{1}{c|}{\cellcolor[HTML]{CCCCCC}SIG ASR} & ACC \\ \midrule
%     No Defense & \multicolumn{1}{c|}{85.99} & \multicolumn{1}{c|}{86.41} & 84.26 & \multicolumn{1}{c|}{91.40} & \multicolumn{1}{c|}{89.49} & 84.06 & \multicolumn{1}{c|}{96.26} & \multicolumn{1}{c|}{90.27} & 84.32 \\ \hline
%     \rowcolor[HTML]{EFEFEF} 
%     Ours & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}6.16} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}5.24} & 81.94 & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}1.70} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}3.44} & 80.65 & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}2.89} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}4.20} & 81.76 \\ \hline
%     NPD & \multicolumn{1}{c|}{1250} & \multicolumn{1}{c|}{1000} & - & \multicolumn{1}{c|}{1250} & \multicolumn{1}{c|}{1000} & - & \multicolumn{1}{c|}{1250} & \multicolumn{1}{c|}{1000} & - \\ \hline
%     NFD & \multicolumn{1}{c|}{55} & \multicolumn{1}{c|}{55} & - & \multicolumn{1}{c|}{55} & \multicolumn{1}{c|}{55} & - & \multicolumn{1}{c|}{55} & \multicolumn{1}{c|}{55} & - \\ \hline
%     PoiNum & \multicolumn{1}{c|}{0} & \multicolumn{1}{c|}{0} & - & \multicolumn{1}{c|}{0} & \multicolumn{1}{c|}{0} & - & \multicolumn{1}{c|}{0} & \multicolumn{1}{c|}{0} & - \\ \bottomrule
%     \end{tabular}
%     }
% \end{table}

























% \begin{table}[]
%     \caption{
%     Performance of T-Core in a \textbf{realistic transfer learning scenario} with 200 samples per class from CIFAR-10. We set the initial seed rate to 20\%, expand it to 30\% during seed expansion, and proceed with the remaining T-Core steps. \review{B}{Q10}
%     }
%     \resizebox{0.47\textwidth}{!}{\large
%     \begin{tabular}{c|cccc|cc}
%     \toprule
%     \rowcolor[HTML]{CCCCCC} 
%     \cellcolor[HTML]{CCCCCC} & \multicolumn{4}{c|}{\cellcolor[HTML]{CCCCCC}\threattwo} & \multicolumn{2}{c}{\cellcolor[HTML]{CCCCCC}\threatthree} \\ \cline{2-7} 
%     \rowcolor[HTML]{CCCCCC} 
%     \cellcolor[HTML]{CCCCCC} & \multicolumn{2}{c|}{\cellcolor[HTML]{CCCCCC}Blended} & \multicolumn{2}{c|}{\cellcolor[HTML]{CCCCCC}SIG} & \multicolumn{2}{c}{\cellcolor[HTML]{CCCCCC}DRUPE} \\ \cline{2-7} 
%     \rowcolor[HTML]{CCCCCC} 
%     \multirow{-3}{*}{\cellcolor[HTML]{CCCCCC}\begin{tabular}[c]{@{}c@{}}Dataset\\ Poisoning\end{tabular}} & ACC$\uparrow$ & \multicolumn{1}{c|}{\cellcolor[HTML]{CCCCCC}ASR$\downarrow$} & ACC$\uparrow$ & ASR$\downarrow$ & ACC$\uparrow$ & ASR$\downarrow$ \\ \midrule
%     No Defense & 62.00 & \multicolumn{1}{c|}{40.61} & 62.83 & 57.58 & 63.54 & 99.82 \\ \hline
%     Ours & 56.44 & \multicolumn{1}{c|}{3.25} & 55.56 & 4.99 & 55.97 & 1.51 \\ \bottomrule
%     \end{tabular}
%     }
%     \end{table}



% \begin{table}[]
%     \caption{Ablation on the \textbf{number of layers} in the classification head of our end-to-end T-Core.
%     For this experiment, we use an STL-10 encoder and a data poisoning attack of SIG on CIFAR-10. \review{D}{Q16}
%     }
%     \resizebox{0.4\textwidth}{!}{\large
%     \begin{tabular}{c|cc|cc}
%     \toprule
%     \rowcolor[HTML]{BFBFBF} 
%     \cellcolor[HTML]{BFBFBF} & \multicolumn{2}{c|}{\cellcolor[HTML]{BFBFBF}No Defense} & \multicolumn{2}{c}{\cellcolor[HTML]{BFBFBF}T-Core} \\ \cline{2-5} 
%     \rowcolor[HTML]{BFBFBF} 
%     \multirow{-2}{*}{\cellcolor[HTML]{BFBFBF}Num of Layers} & \multicolumn{1}{c|}{\cellcolor[HTML]{BFBFBF}ASR} & ACC & \multicolumn{1}{c|}{\cellcolor[HTML]{BFBFBF}ASR} & ACC \\ \midrule
%     3 & \multicolumn{1}{c|}{89.10} & 84.72 & \multicolumn{1}{c|}{2.54} & 87.31 \\ \hline
%     5 & \multicolumn{1}{c|}{90.80} & 84.60 & \multicolumn{1}{c|}{3.25} & 86.79 \\ \hline
%     7 & \multicolumn{1}{c|}{88.49} & 84.09 & \multicolumn{1}{c|}{3.18} & 85.94 \\ \bottomrule
%     \end{tabular}
%     }
% \end{table}

\begin{table*}[htbp]
    \centering
    % 第一个minipage
    \begin{minipage}[t]{0.48\textwidth}
        \centering
        \caption{
        Performance of T-Core in a \textbf{realistic transfer learning scenario} with 200 samples per class from CIFAR-10. We set the initial seed rate to 20\%, expand it to 30\% during seed expansion, and proceed with the remaining T-Core steps. \review{B}{Q10}
        }
        \vspace{10pt}
        \resizebox{\textwidth}{!}{\large
        \begin{tabular}{c|cccc|cc}
        \toprule
        \rowcolor[HTML]{FFFFFF} 
        \cellcolor[HTML]{FFFFFF} & \multicolumn{4}{c|}{\cellcolor[HTML]{FFFFFF}\threattwo} & \multicolumn{2}{c}{\cellcolor[HTML]{FFFFFF}\threatthree} \\ \cline{2-7} 
        \rowcolor[HTML]{FFFFFF} 
        \cellcolor[HTML]{FFFFFF} & \multicolumn{2}{c|}{\cellcolor[HTML]{FFFFFF}Blended} & \multicolumn{2}{c|}{\cellcolor[HTML]{FFFFFF}SIG} & \multicolumn{2}{c}{\cellcolor[HTML]{FFFFFF}DRUPE} \\ \cline{2-7} 
        \rowcolor[HTML]{FFFFFF} 
        \multirow{-3}{*}{\cellcolor[HTML]{FFFFFF}\begin{tabular}[c]{@{}c@{}}Dataset\\ Poisoning\end{tabular}} & ACC$\uparrow$ & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}ASR$\downarrow$} & ACC$\uparrow$ & ASR$\downarrow$ & ACC$\uparrow$ & ASR$\downarrow$ \\ \midrule
        No Defense & 62.00 & \multicolumn{1}{c|}{40.61} & 62.83 & 57.58 & 63.54 & 99.82 \\ \hline
        Ours & 56.44 & \multicolumn{1}{c|}{3.25} & 55.56 & 4.99 & 55.97 & 1.51 \\ \bottomrule
        \end{tabular}
        }
    \end{minipage}
    \hfill % 添加水平间距
    % 第二个minipage
    \begin{minipage}[t]{0.48\textwidth}
        \centering
        \caption{Ablation on the \textbf{number of layers} in the classification head of our end-to-end T-Core.
        For this experiment, we use an STL-10 encoder and a data poisoning attack of SIG on CIFAR-10. \review{D}{Q16}
        }
        \resizebox{\textwidth}{!}{\large
        \begin{tabular}{c|cc|cc}
        \toprule
        \rowcolor[HTML]{BFBFBF} 
        \cellcolor[HTML]{BFBFBF} & \multicolumn{2}{c|}{\cellcolor[HTML]{BFBFBF}No Defense} & \multicolumn{2}{c}{\cellcolor[HTML]{BFBFBF}T-Core} \\ \cline{2-5} 
        \rowcolor[HTML]{BFBFBF} 
        \multirow{-2}{*}{\cellcolor[HTML]{BFBFBF}Num of Layers} & \multicolumn{1}{c|}{\cellcolor[HTML]{BFBFBF}ASR} & ACC & \multicolumn{1}{c|}{\cellcolor[HTML]{BFBFBF}ASR} & ACC \\ \midrule
        3 & \multicolumn{1}{c|}{89.10} & 84.72 & \multicolumn{1}{c|}{2.54} & 87.31 \\ \hline
        5 & \multicolumn{1}{c|}{90.80} & 84.60 & \multicolumn{1}{c|}{3.25} & 86.79 \\ \hline
        7 & \multicolumn{1}{c|}{88.49} & 84.09 & \multicolumn{1}{c|}{3.18} & 85.94 \\ \bottomrule
        \end{tabular}
        }
    \end{minipage}
\end{table*}



\begin{table*}[]
    \caption{Performance of the state-of-the-art \textbf{inference-time defenses} SCALE-UP and IBD-PSC under different threat scenarios, using the CIFAR-10 dataset. \review{C}{Q11}
    }
    \resizebox{\textwidth}{!}{\large
    \begin{tabular}{c|c|cccc|cccc}
    \toprule
    \rowcolor[HTML]{FFFFFF} 
    \cellcolor[HTML]{FFFFFF} & \cellcolor[HTML]{FFFFFF} & \multicolumn{4}{c|}{\cellcolor[HTML]{FFFFFF}SCALE-UP} & \multicolumn{4}{c}{\cellcolor[HTML]{FFFFFF}IBD-PSC} \\ \cline{3-10} 
    \rowcolor[HTML]{FFFFFF} 
    \multirow{-2}{*}{\cellcolor[HTML]{FFFFFF}Threat Type} & \multirow{-2}{*}{\cellcolor[HTML]{FFFFFF}\begin{tabular}[c]{@{}c@{}}Dataset\\ Poisoning\end{tabular}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}TPR(\%)$\uparrow$} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}FPR(\%)$\downarrow$} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}AUC$\uparrow$} & F1 $\uparrow$& \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}TPR(\%)$\uparrow$} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}FPR(\%)$\downarrow$} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}AUC$\uparrow$} & F1$\uparrow$ \\ \midrule
     & BadNets & \multicolumn{1}{c|}{92.80} & \multicolumn{1}{c|}{33.98} & \multicolumn{1}{c|}{0.79} & 0.12 & \multicolumn{1}{c|}{0.00} & \multicolumn{1}{c|}{3.38} & \multicolumn{1}{c|}{0.48} & 0.00 \\ \cline{2-10} 
     & Blended & \multicolumn{1}{c|}{20.24} & \multicolumn{1}{c|}{38.22} & \multicolumn{1}{c|}{0.41} & 0.03 & \multicolumn{1}{c|}{0.24} & \multicolumn{1}{c|}{3.27} & \multicolumn{1}{c|}{0.48} & 0.00 \\ \cline{2-10} 
     & SIG & \multicolumn{1}{c|}{14.80} & \multicolumn{1}{c|}{37.66} & \multicolumn{1}{c|}{0.39} & 0.02 & \multicolumn{1}{c|}{0.80} & \multicolumn{1}{c|}{3.13} & \multicolumn{1}{c|}{0.49} & 0.01 \\ \cline{2-10} 
     & WaNet & \multicolumn{1}{c|}{28.56} & \multicolumn{1}{c|}{40.07} & \multicolumn{1}{c|}{0.44} & 0.03 & \multicolumn{1}{c|}{4.80} & \multicolumn{1}{c|}{0.42} & \multicolumn{1}{c|}{0.52} & 0.08 \\ \cline{2-10} 
     & TaCT & \multicolumn{1}{c|}{56.88} & \multicolumn{1}{c|}{35.98} & \multicolumn{1}{c|}{0.60} & 0.07 & \multicolumn{1}{c|}{0.00} & \multicolumn{1}{c|}{5.29} & \multicolumn{1}{c|}{0.47} & 0.00 \\ \cline{2-10} 
     & Adap-Blend & \multicolumn{1}{c|}{29.60} & \multicolumn{1}{c|}{35.54} & \multicolumn{1}{c|}{0.47} & 0.04 & \multicolumn{1}{c|}{0.80} & \multicolumn{1}{c|}{4.14} & \multicolumn{1}{c|}{0.48} & 0.01 \\ \cline{2-10} 
    \multirow{-7}{*}{\threattwo} & Adap-Patch & \multicolumn{1}{c|}{32.48} & \multicolumn{1}{c|}{34.58} & \multicolumn{1}{c|}{0.49} & 0.04 & \multicolumn{1}{c|}{1.92} & \multicolumn{1}{c|}{2.28} & \multicolumn{1}{c|}{0.50} & 0.02 \\ \midrule
    \rowcolor[HTML]{FFFFFF} 
    Threat Type & \begin{tabular}[c]{@{}c@{}}Encoder\\ Poisioning\end{tabular} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}TPR(\%)$\uparrow$} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}FPR(\%)$\downarrow$} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}AUC$\uparrow$} & F1$\uparrow$ & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}TPR(\%)$\uparrow$} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}FPR(\%)$\downarrow$} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}AUC$\uparrow$} & F1$\uparrow$ \\ \midrule
     & BadEncoder & \multicolumn{1}{c|}{33.60} & \multicolumn{1}{c|}{37.00} & \multicolumn{1}{c|}{0.48} & 0.04 & \multicolumn{1}{c|}{3.76} & \multicolumn{1}{c|}{4.59} & \multicolumn{1}{c|}{0.50} & 0.03 \\ \cline{2-10} 
    \multirow{-2}{*}{\threatone} & Dpure & \multicolumn{1}{c|}{33.84} & \multicolumn{1}{c|}{36.90} & \multicolumn{1}{c|}{0.48} & 0.04 & \multicolumn{1}{c|}{0.24} & \multicolumn{1}{c|}{3.93} & \multicolumn{1}{c|}{0.48} & 0.00 \\ \hline
     & BadEncoder & \multicolumn{1}{c|}{53.04} & \multicolumn{1}{c|}{38.60} & \multicolumn{1}{c|}{0.57} & 0.06 & \multicolumn{1}{c|}{50.64} & \multicolumn{1}{c|}{3.96} & \multicolumn{1}{c|}{0.73} & 0.33 \\ \cline{2-10} 
    \multirow{-2}{*}{\threatthree} & Dpure & \multicolumn{1}{c|}{51.76} & \multicolumn{1}{c|}{34.18} & \multicolumn{1}{c|}{0.59} & 0.07 & \multicolumn{1}{c|}{3.76} & \multicolumn{1}{c|}{6.98} & \multicolumn{1}{c|}{0.48} & 0.02 \\ \bottomrule
    \end{tabular}
    }
\end{table*}






% \begin{lstlisting}


% \end{lstlisting}

